Pre-trained Embeddings for Entity Resolution: An Experimental Analysis [Experiment, Analysis & Benchmark]

Many recent works on Entity Resolution (ER) leverage Deep Learning techniques involving language models to improve effectiveness. This is applied to both main steps of ER, i.e., blocking and matching. Several pre-trained embeddings have been tested, with the most popular ones being fastText and variants of the BERT model. However, there is no detailed analysis of their pros and cons. To cover this gap, we perform a thorough experimental analysis of 12 popular language models over 17 established benchmark datasets. First, we assess their vectorization overhead for converting all input entities into dense embeddings vectors. Second, we investigate their blocking performance, performing a detailed scalability analysis, and comparing them with the state-of-the-art deep learning-based blocking method. Third, we conclude with their relative performance for both supervised and unsupervised matching. Our experimental results provide novel insights into the strengths and weaknesses of the main language models, facilitating researchers and practitioners to select the most suitable ones in practice.

==> blocking.tex <==
\section{Performance Comparison on Blocking}
\label{sec:blocking}

Blocking receives as input the vectorized entities of the given datasets and returns as output a set of candidate pairs.
% , i.e., pairs of entities that are highly likely to be matching.
To assess 
% the performance We now examine
the performance of the language models on blocking, we again consider all 
% the task of schema-agnostic blocking. 
% To this end, we use the datasets in Table \ref{tb:rlDatasets} in schema-agnostic settings. 
% For each 
datasets in Table \ref{tb:datasets}(a).
% Since the size of the datasets is relatively small, we perform exact nearest neighbor search.

%We first index the vectorized entities of Dataset${_1}$ using FAISS \cite{DBLP:journals/tbd/JohnsonDJ21} in combination with HNSW \cite{DBLP:journals/pami/MalkovY20}. Then, we query the resulting index with every vectorized entity of Dataset${_2}$, retrieving $k \in \{1, 5, 10\}$ candidates per query. FAISS(HNSW) is a state-of-the-art algorithm for nearest neighbor search, exhibiting one of the highest throughput in answering queries~\cite{DBLP:journals/is/AumullerBF20}. {\color{red}To maximize effectiveness, we used its exact search mode, which returns the actual nearest neighbors, without leveraging any approximations.}



\begin{figure*}[!t]
\centering
\subfloat[D1 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D1_Recall.pdf}} 
\subfloat[D1 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D1_Time.pdf}}
\subfloat[D2 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D2_Recall.pdf}} 
\subfloat[D2 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D2_Time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D3 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D3_Recall.pdf}} 
\subfloat[D3 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D3_Time.pdf}}
\subfloat[D4 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D4_Recall.pdf}} 
\subfloat[D4 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D4_Time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D5 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D5_Recall.pdf}} 
\subfloat[D5 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D5_Time.pdf}}
\subfloat[D6 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D6_Recall.pdf}} 
\subfloat[D6 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D6_Time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D7 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D7_Recall.pdf}} 
\subfloat[D7 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D7_Time.pdf}}
\subfloat[D8 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D8_Recall.pdf}} 
\subfloat[D8 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D8_Time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D9 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D9_Recall.pdf}} 
\subfloat[D9 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D9_Time.pdf}}
\subfloat[D10 / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D10_Recall.pdf}} 
\subfloat[D10 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/blocking_real_D10_Time.pdf}}
\vspace{-12pt}
\caption{Recall and Blocking Time (sec) per method from real data per case. There are three values for $k \in \{${\color{myblue}1}, {\color{myorange}5}, {\color{mygreen}10} $\}$.}
\vspace{-12pt}
\label{fig:blk_real}
\end{figure*}

\subsection{Effectiveness}

% To assess the effectiveness of the resulting candidate pairs, we measure their recall,
We measure the recall of the resulting candidate pairs, 
which is also known as pairs completeness \cite{DBLP:journals/is/KenigG13,DBLP:journals/tkde/Christen12,DBLP:journals/pvldb/0001APK15}.
% Pairs Quality $PQ$ (i.e., precision) 
Recall is the most critical evaluation measure for blocking, as it typically sets the upper bound for the subsequent matching step, i.e., a low blocking recall usually yields even lower matching recall, unless complex and time-consuming iterative algorithms are employed \cite{DBLP:journals/pvldb/GetoorM12,DBLP:books/daglib/0030287}. In contrast, precision is typically low after blocking, due to the large number of false positives, but significantly raises after matching. {\color{blue}In more detail, in blocking, for each query entity we search for its nearest $k$ neighbors. Thus, in terms of precision, all models have the same denominator (i.e. total number of candidates) and precision can be omitted, since recall and precision behave the same.}
% We omit precision here, because all models have the same denominator (i.e., total number of candidates), due to the same $k$ per query entity, thus recall and precision behave the same.

%We omit precision here, because all models have the same denominator (i.e., total number of candidates), due to the same $k$ per query entity, thus recall and precision behave the same.


% Note, though, that we disregard precision (a.k.a., pairs quality), because all models have practically the same denominator (i.e., total number of candidates), due to the same $k$ per query entity. In other words, the precision of the considered models differs only in the numerator, which is the same as in recall. As a result, recall and precision have the same behavior in the settings we are considering and, thus, we omit the latter for brevity.

The experimental outcomes are shown in Figure \ref{fig:blk_real}. For all models, the recall increases with higher $k$ across all datasets, which is expected, given that the set of candidate pairs gets larger. The same applies to the query time, due to the larger number of neighbors that are retrieved.
% There are also several interesting patterns in the behavior of each model.
More specifically:

% {\color{red} as regards the schema-agnostic settings. Note that we used..}
% \textbf{Schema-agnostic settings.} We represent every entity through a sentence that concatenates all its attribute values and is then vectorized by each model. 
% The corresponding performance per dataset and model appears in Figure \ref{fig:blk_real}. 

$\bullet$ The SentenceBERT models consistently achieve the highest recall among all considered models. Among them, S-DistilRoBERTa is the least effective, followed in close distance by SMPNet, while ST-5 takes the lead in all datasets, leaving S-MiniLM in the second place. This applies to all values of $k$.
% Indeed, 
The average recall of S-DistilRoBERTa, SMPNet, S-MiniLM and ST-5
% amounts to 0.788, 0.796, 0.823 and 0.847, respectively, for $k$=1, increasing to 0.885, 0.896, 0.904 and 0.923 for $k$=5 and to 0.902, 0.913, 0.920 and 0.937 for $k$=10. Hence, their performance
is quite high in all datasets, except $D_{10}$, which abounds in noisy and missing values. In $D_{10}$, all SentenceBERT models actually exhibit a recall $\sim$0.55 for $k=10$, which is the highest among all models. Excluding $D_{10}$, the average recall of all SentenceBERT models fluctuates between 0.960 (S-DistilRoBERTa) and 0.997 (ST-5).
% , which indicates perfect recall.
Their recall is also quite robust, with a standard deviation lower than 0.04 for all models.

$\bullet$ On the other extreme lie AlBERT and XLNet, which consistently underperform all other models. Their average recall across the datasets $D_1$-$D_9$ for $k$=10 is just 0.261 and 0.193, respectively. The situation is worse over $D_{10}$, where their recall is consistently lower than 0.05.
% This means that both language models are not suitable for blocking.

$\bullet$ The second best group of models are the static ones. They exhibit large differences between them for $k$=1 and $k$=5, but converge to quite similar recall for $k$=10. In all cases, though, GloVe is the top performer, with FastText and Word2Vec in the second and third place, respectively.
% On average, excluding $D_{10}$, recall amounts to 0.563, 0.682 and 0.720 for Word2Vec, to 0.612, 0.698 and 0.728 for FastText and to 0.639, 0.733 and 0.770 for GloVe for $k$=1, 5 and 10, respectively.
In $D_{10}$, though, their relative performance is quite different: FastText does not exceed 0.10, GloVe remains lower than 0.17, while Word2Vec ranges from 0.26 ($k$=1) to 0.36 ($k$=10).
% {\color{red}This means that Word2Vec is more capable of addressing the ambiguity and noise in $D_{10}$, due to the datasets used in its training.}

$\bullet$ The remaining BERT-based models underperform all static pre-trained ones in almost all cases. Among them, DistilBERT is the top performer.
% , with an average recall of 0.571 and 0.616 for $k$=5 and $k$=10.
BERT lies in the second place, but its advantage over RoBERTa is
% {\color{red}statistically insignificant}.
not significant. Their difference in terms of average recall is less than 2\% in all cases.
% : 0.423 (BERT) vs 0.440 (RoBERTa) for $k$=1, 0.522 vs 0.519 for $k$=5 and 0.562 vs 0.544 for $k$=10.
In the case of $D_{10}$, all these models achieve rather poor recall, which is lower than 0.035 even for $k$=10.

\textbf{Summary.} 
% {\color{red}George: The rest will be extended.
% These patterns are summarized in 
%Overall, the relative performance of the blocking methods is summarized in 
Figure \ref{fig:blk_heat}
% , which 
reports the ranking of each model per dataset with respect to recall for $k$=10. Looking at the rightmost column, which indicates the average position per model, 
% the \textit{blocking f-measure} ($BF1$), i.e., the harmonic mean of blocking recall and blocking precision.
we observe that the first four places are occupied by the SentenceBERT models, with ST-5 ranking first in most datasets and second in the rest. It is interesting that none of these models falls below the fourth place. The next three ranking positions correspond to the static models, with Word2Vec having the highest average one. Yet, FastText is the most stable one, fluctuating between positions 5 and 7, unlike the other two models, which fall up to the 10$^{th}$ place. Finally, BERT-based models are mapped to the last five positions. DistilBERT is the best one, ranked 8$^{th}$ on average, while AlBERT and XLNet are constantly ranked 11$^{th}$ and 12$^{th}$, respectively.
% }

These patterns suggest a high correlation in terms of effectiveness between the models that belong to the same category. Indeed, the Pearson correlation with respect to recall for $k$=10 between the models of each category is quite high ($\geq0.9)$, as shown in Figure \ref{fig:blk_heat_pear}. The correlation is equally high between the pre-trained static models and the SentenceBERT ones, due to the high performance of both categories. In contrast, the correlation between BERT-based and the other two categories is significantly lower: it fluctuates between 0.58 and 0.85 for the SentenceBERT models and between 0.69 and 0.86 for the static ones. In the latter case, DistilBERT is an exception, fluctuating between 0.84 and and 0.94, since it is the best-performing BERT model and, thus, it is closer to the static~ones. 

% \begin{figure*}[!t]
% \centering
% \subfloat[Schema-based]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.47\textwidth]{figures/blocking_real_vec_exact_sch_heat.pdf}\label{subfig:blk_heat_sch}}
% \subfloat[Schema-agnostic]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.47\textwidth]{figures/blocking_real_vec_exact_agn_heat.pdf}\label{subfig:blk_heat_agn}}
% \vspace{-5pt}
% \caption{The ranking position of each method for $BF1$ per dataset in (a) schema-agnostic
% and (b) schema-based settings for Blocking for $k=10$. Lower is better. {\color{red}Check this}}
% \label{fig:blk_heat}
% \end{figure*}

\begin{figure}[!t]
\centering
\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_agn_heat.pdf}
\vspace{-12pt}
% \caption{The ranking position of each method with respect to blocking recall per dataset. Lower is better.}
\caption{Method ranking wrt blocking recall (lower is better).}
\vspace{-12pt}
\label{fig:blk_heat}
\end{figure}

% In more detail, the highest precision corresponds to the SentenceBERT models. On average, excluding $D_{10}$, it is very high for $k=1$ ($\sim$0.280), but decreases for higher $k$, i.e., 0.065 for $k=5$ and 0.033 for $k=10$. These models are followed by the static pre-trained ones, which start from $\sim$0.200 ($k=1$) and drop to $\sim$0.050 and $\sim$0.025 for $k=5$ and $k=10$, respectively. For AlBERT and XLNet, $PQ$ is lower than 0.05 in practically all cases, while for the rest of the BERT-based models, it goes from $\sim$0.140 for $k=1$ to $\sim$0.035 and $\sim$0.020 for $k=5$ and $k=10$, respectively.

\subsection{Efficiency}

% To assess the time efficiency of blocking, we measure the 
% execution time.
% overhead time $t_o$, which consists of the indexing and querying time.
The execution time of blocking is very low for all models, not exceeding 0.5 seconds in most cases. The only exceptions are the two largest datasets, $D_9$ and $D_{10}$, which still require less than 2 seconds in all cases. The differences between the various models are rather insignificant.
% , as $t_v$ does not include the vectorization time.
Yet, there are significant differences among the values of $k$ 
% number of candidates 
we have considered.
% More specifically, excluding $D_9$ and $D_{10}$, the average run-time of all models fluctuates between 54 and 138 msec for $k$=1, 63 and 149 msec for $k$=5 and 78 and 163 msec for $k$=10.
In most cases, the lower end in these ranges corresponds to the language models with the lowest dimensionality, namely the static ones (300) as well as S-MiniLM (385), and the higher end to the rest of the models, which involve 768-dimensional vectors (see Table \ref{tb:modelCharacteristics}).
In more detail, fastText and S-T5 are consistently the fastest and slowest models, respectively. However, this overhead time is negligible in comparison to the vectorization time in Table \ref{tb:vectTime}. For this reason, the relative time efficiency remains the same as the one discussed in Section \ref{sec:vectorizonExp}.
% {\color{red}[Dimitris: This time relates to the dimensionality of the vectors, right? If, so, we I guess we should show/comment on this.]}

\begin{figure}[!t]
\centering
\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.47\textwidth]{figures/blocking_real_vec_exact_agn_corr.pdf}
\vspace{-12pt}
% \caption{{\small Pearson correlation per pair of models wrt blocking~recall.}}
\caption{Pearson correlation of models wrt blocking recall.}
\label{fig:blk_heat_pear}
\vspace{-8pt}
\end{figure}

\input{tables/st5VsDeepBlocker}

% \textbf{Comparison to DeepBlocker.}

\begin{figure*}[!t]
\centering
\subfloat{\includegraphics[width=1.0\linewidth]{figures/blocking_synthetic_legend.pdf}}
\vspace{-7pt}
\setcounter{subfigure}{0}
% \newline
\subfloat[Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_recall_approx.pdf}\label{subfig:blk_synth_rec_app}}
\subfloat[Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_precision_approx.pdf}\label{subfig:blk_synth_pre_app}}
\subfloat[Blocking Time (sec-log)]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_time_approx.pdf}\label{subfig:blk_synth_time_app}}
\subfloat[Vectorization  Time (sec-log)]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/vectorization_synthetic_time.pdf}\label{subfig:vec_synth_time}}
% \subfloat[Memory]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_synthetic_memory.pdf}\label{subfig:vec_synth_memory}}

\vspace{-12pt}
\caption{Scalability analysis over the synthetic datasets in Table \ref{tb:datasets}(b). The horizontal axis indicates the number of input entities.}
\label{fig:blk_synth}
\vspace{-15pt}
\end{figure*}

\subsection{Comparison to state-of-the-art}

We now compare the best performing language model, S-T5, with the state-of-the-art blocking approach that is based on deep learning and embeddings vectors: DeepBlocker's Auto-Encoder with FastText embeddings. The relative performance of the two methods over all datasets in Table \ref{tb:datasets}(a) appears in Table \ref{tb:st5vsdeepblocker} (including vectorization time for S-T5). Note that since DeepBlocker is a stochastic approach, we take the average of 10 runs.

\textbf{Effectiveness.}
S-T5 consistently outperforms DeepBlocker's recall to a significant extent. The only exceptions are $D_1$ and $D_4$, where both methods achieve practically perfect recall -- except for $k=1$, where S-T5 is marginally better, by 3\% and 1\%, respectively. The reason is that $D_1$ involves a very low number of duplicate pairs in relation to the size of each data source, while $D_4$ contains relatively clean entities with long textual descriptions that are easy to match.
In the remaining 8 datasets, the superiority of S-T5 is inversely proportional to the number of candidates per query entity, i.e., the lower $k$ is, the larger is the advantage of S-T5.
% For $k$=1, the recall of S-T5 is higher than DeepBlocker from 11.5\% ($D_6$) to 50.7\% ($D_2$), with an average of 31.3\%; for $k$=5, their differences fluctuate from 5.1\% ($D_6$) to 38.5\% ($D_2$), with a mean of 21.6\%, and for $k$=10, it is higher from 3.1\% ($D_6$) to 35.4\% ($D_2$), with an average of 18.8\%.

\textbf{Efficiency.}
% In terms of time efficiency, 
DeepBlocker is consistently faster than S-T5 for $k$=1 and $k$=5 in all datasets but $D_{10}$.
% In fact, the blocking time of DeepBlocker is lower than S-T5 from 36\%	($D_1$) to 60.6\% ($D_3$) with an average of 49.5\% for both $k$=1 and $k$=5.
The reason for the slow operation of S-T5 is its high vectorization cost, which accounts for $\sim$99\% of the overall blocking time. This explains why its run-time is practically stable per dataset across all values of $k$. This is expected, though, given that S-T5 leverages 768-dimensional embeddings vectors, compared to 300-dimensional FastText vectors of DeepBlocker. Yet, for $k$=10, DeepBlocker is faster than S-T5 only in $D_2$ and $D_3$ (by 14.4\% and 26\%, respectively). The situation is reversed in $D_1$ and $D_4$-$D_8$, where S-T5 is faster by 14.1\%, on average. The reason is that DeepBlocker does not scale well as the number of candidates per query entity increases, due to the high complexity of the deep neural network that lies at its core. Most importantly, DeepBlocker does scale well as the size of the input data increases: in $D_{10}$, S-T5 is faster by 1.5 times for $k \in \{1, 5\}$ and 3.7 times for $k$=10. This is further verified in Section~\ref{sec:scalability}.

\textbf{Summary.} 
Overall, we can conclude that S-T5 exhibits much higher blocking recall than DeepBlocker in all non-trivial cases at the cost of much higher overhead in case of small datasets and few candidates per query entity. In all other cases, S-T5 dominates DeepBlocker with respect to both effectiveness and time efficiency.


% \textbf{Schema-based settings.} In this case, we vectorize the input entities by considering the values specific attributes. {\color{red}These attributes are reported in Table \ref{tb:rlDatasets}.} For brevity, we omit the detailed performance in terms of precision, recall and overhead time. Instead, Figure \ref{fig:blk_heat}(b) presents the ranking of models per dataset and in the average case in terms of F1, i.e., the harmonic mean of recall (recall) and $PQ$ (precision).


% \begin{table}[]
% \caption{Columns selected for schema-based blocking.}
% \vspace{-5pt}
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% Case & Dataset1 & Dataset2 & Attribute D1 & Attribute D2 \\ \hline
% D1 & Rest.1 & Rest.2 & name & phone\_number \\ \hline
% D2 & Abt & Buy & name & description \\ \hline
% D3 & Amazon & Google & title & description \\ \hline
% D4 & DBLP & Pr. ACM & title & authors \\ \hline
% D5 & IMDb & TMDb & title & name \\ \hline
% D6 & IMDb & TVDB & title & name \\ \hline
% D7 & TMDb & TVDB & title & name \\ \hline
% D8 & Walmart & Amazon & title & modelno \\ \hline
% D9 & DBLP & Scholar & title & authors \\ \hline
% D10 & IMDb & DBpedia & title & starring / actor name \\ \hline
% \end{tabular}
% \label{tab:schema_based}
% \end{table}

% \noindent \textbf{How each case performs} Results in Fig \ref{fig:blk_case} and Table \ref{tab:schema_based}.

% \begin{figure*}[!t]
% \centering
% \subfloat[Schema-Based Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_case_sch.pdf}\label{subfig:blk_case_sch}}
% \subfloat[Schema-Agnostic Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_case_agn.pdf}\label{subfig:blk_case_agn}}
% \newline
% \subfloat[Schema-Based Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_case_sch2.pdf}\label{subfig:blk_case_sch2}}
% \subfloat[Schema-Agnostic Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_case_agn2.pdf}\label{subfig:blk_case_agn2}}
% \caption{Blocking Statistics from real data per case.}
% \label{fig:blk_case}
% \end{figure*}

% \noindent \textbf{How each vectorizer performs} Results in Fig \ref{fig:blk_vec}.

% \begin{figure*}[!t]
% \centering
% \subfloat[Schema-Based Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_vec_sch.pdf}\label{subfig:blk_vec_sch}}
% \subfloat[Schema-Agnostic Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_vec_agn.pdf}\label{subfig:blk_vec_agn}}
% \newline
% \subfloat[Schema-Based Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_vec_sch2.pdf}\label{subfig:blk_vec_sch2}}
% \subfloat[Schema-Agnostic Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_exact_vec_agn2.pdf}\label{subfig:blk_vec_agn2}}
% \caption{Blocking Statistics from real data per vectorizer.}
% \label{fig:blk_vec}
% \end{figure*}

% \noindent \textbf{How does a-NNS compare to exact} Results in Fig \ref{fig:blk_app}.

% \begin{figure*}[!t]
% \centering
% % \subfloat[Exact / Schema-Based]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_sch.pdf}\label{subfig:blk_vec_sch}}
% % \subfloat[Exact / Schema-Agnostic]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_agn.pdf}\label{subfig:blk_vec_agn}}
% % \newline
% \subfloat[Schema-Based]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_app_sch.pdf}\label{subfig:blk_vec_sch}}
% \subfloat[Schema-Agnostic]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_app_agn.pdf}\label{subfig:blk_vec_agn}}
% \caption{Blocking Statistics from real data per vectorizer (approximate).}
% \label{fig:blk_app}
% \end{figure*}

% \begin{figure*}[!t]
% \centering
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.3\linewidth]{figures/blocking_real_legend.pdf}}
% \setcounter{subfigure}{0}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D1_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D1_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D1_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D2_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D2_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D2_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D3_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D3_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D3_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D4_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D4_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D4_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D5_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D5_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D5_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D6_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D6_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D6_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D7_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D7_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D7_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D8_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D8_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D8_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D9_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D9_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D9_Time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D10_Precision.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D10_Recall.pdf}} \hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/blocking_real_D10_Time.pdf}}
% \newline
% \caption{Precision, Recall and Blocking Time per k and per method from real data per case.}
% \label{fig:blk_real}
% \end{figure*}



% \begin{figure*}[!t]
% \centering
% \subfloat[Schema-based]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_sch_corr.pdf}\label{subfig:blk_heat_sch}}
% \subfloat[Schema-agnostic]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_agn_corr.pdf}\label{subfig:blk_heat_agn}}

% \caption{The correlation per pair of vectorizers for F1 for (a) schema-agnostic
% and (b) schema-based settings for Blocking.}
% \label{fig:blk_heat}
% \end{figure*}






% \begin{figure*}[!t]
% \centering
% \subfloat[Exact / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_synthetic_recall_exact.pdf}\label{subfig:blk_synth_rec_ex}}
% \subfloat[Approximate / Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_synthetic_recall_approx.pdf}\label{subfig:blk_synth_rec_app}}
% \newline
% \subfloat[Exact / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_synthetic_time_exact.pdf}\label{subfig:blk_synth_time_ex}}
% \subfloat[Approximate / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_synthetic_time_approx.pdf}\label{subfig:blk_synth_time_app}}
% \caption{Blocking Statistics from synthetic data per case}
% \label{fig:blk_synth}
% \end{figure*}


==> blocking_2.tex <==
\section{Performance Comparison on Blocking}
\label{sec:blocking}

Blocking receives as input the vectorized entities of the given datasets and returns as output a set of candidate pairs.
To assess the performance of the language models on blocking, we again consider all datasets in Table \ref{tb:datasets}(a).

\begin{figure*}[!t]
\centering
\subfloat[Static]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/blocking_static.pdf}} 
\subfloat[BERT]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/blocking_BERT.pdf}}
\subfloat[SBERT]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/blocking_SBERT.pdf}} 
\caption{Recall in Blocking per group of methods from real data (k=10).}
\vspace{-12pt}
\label{fig:blk_rec_real}
\end{figure*}

% \begin{figure}[!t]
% \centering
% \includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.50\textwidth]{figures/blocking_pareto.pdf} 
% \caption{Pareto Front for Recall and Blocking Time (sec) per method from real data (k=10).}
% \vspace{-12pt}
% \label{fig:blk_time_real}
% \end{figure}

\subsection{Effectiveness}

We measure the recall of the resulting candidate pairs, 
which is also known as pairs completeness \cite{DBLP:journals/is/KenigG13,DBLP:journals/tkde/Christen12,DBLP:journals/pvldb/0001APK15}.
% Pairs Quality $PQ$ (i.e., precision) 
Recall is the most critical evaluation measure for blocking, as it typically sets the upper bound for the subsequent matching step, i.e., a low blocking recall usually yields even lower matching recall, unless complex and time-consuming iterative algorithms are employed \cite{DBLP:journals/pvldb/GetoorM12,DBLP:books/daglib/0030287}. In contrast, precision is typically low after blocking, due to the large number of false positives, but significantly raises after matching. {\color{blue}In more detail, in blocking, for each query entity we search for its $k$ nearest neighbors. Thus, in terms of precision, all models have the same denominator (i.e. total number of candidates) and precision can be omitted, since recall and precision behave the same.}

The experimental outcomes are shown in Figure \ref{fig:blk_rec_real} for $k=10$ for each category of models.
More specifically:

$\bullet$ In static models, GloVe is the top performer, with FastText and Word2Vec in the second and third place, respectively, except from $D_{10}$, which abounds in noisy and missing values. This seems to confirm the results from bibliography, since GloVe was the latest and more succesful model in the static category.

$\bullet$ In the BERT models, we can see that XLNet and AlBERT have very poor performance on almost all datasets. {\color{red} For XLNet it seems logical, since it was trained for solving PLM, rather than MLM, meaning that it searches for dependency between words and phrases, while in our datasets we have concatenated different columns, producing a possibly not coherent sentence. For AlBERT, since it trains only one encoder to produce a lighter version of BERT and shares its weights with the remaining encoders, if the task in hand can not be efficiently solved by this single encoder - and by not utilizing fine-tuning - then it is clear that it will have a very poor performance, as in our task.} The remaining models have a mediocre performance with DistilBERT probably being the best one in all datasets.

$\bullet$ In the SentenceBERT models, apart from $D_{10}$, all models achieve high recall. The best model in this category is ST-5. {\color{red}missing argument.}

$\bullet$ Finally, between groups, we can see that the point made in \cite{reimers2019sentence} holds in our task as well. BERT models, if not fine-tuned, behave worse in terms of recall than static models (GloVe) and SentenceBERT have overall the best performance.



\textbf{Summary.} 
Figure \ref{fig:blk_heat}
reports the ranking of each model per dataset with respect to recall for $k$=10. Looking at the rightmost column, which indicates the average position per model, 
we observe that the first four places are occupied by the SentenceBERT models, with ST-5 ranking first in most datasets and second in the rest. It is interesting that none of these models falls below the fourth place. The next three ranking positions correspond to the static models, with Word2Vec having the highest average one. Yet, FastText is the most stable one, fluctuating between positions 5 and 7, unlike the other two models, which fall up to the 10$^{th}$ place. Finally, BERT-based models are mapped to the last five positions. DistilBERT is the best one, ranked 8$^{th}$ on average, while AlBERT and XLNet are constantly ranked 11$^{th}$ and 12$^{th}$, respectively.
% }

These patterns suggest a high correlation in terms of effectiveness between the models that belong to the same category. Indeed, the Pearson correlation with respect to recall for $k$=10 between the models of each category is quite high ($\geq0.9)$, as shown in Figure \ref{fig:blk_heat_pear}. The correlation is equally high between the pre-trained static models and the SentenceBERT ones, due to the high performance of both categories. In contrast, the correlation between BERT-based and the other two categories is significantly lower: it fluctuates between 0.58 and 0.85 for the SentenceBERT models and between 0.69 and 0.86 for the static ones. In the latter case, DistilBERT is an exception, fluctuating between 0.84 and and 0.94, since it is the best-performing BERT model and, thus, it is closer to the static~ones. 


\begin{figure}[!t]
\centering
\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/blocking_real_vec_exact_agn_heat.pdf}
\vspace{-12pt}
\caption{Method ranking wrt blocking recall (lower is better).}
\vspace{-12pt}
\label{fig:blk_heat}
\end{figure}


\subsection{Efficiency}

The execution time of blocking is very low for all models, not exceeding 0.5 seconds in most cases. The only exceptions are the two largest datasets, $D_9$ and $D_{10}$, which still require less than 2 seconds in all cases. The differences between the various models are rather insignificant.
In most cases, the lower end in these ranges corresponds to the language models with the lowest dimensionality, namely the static ones (300) as well as S-MiniLM (385), and the higher end to the rest of the models, which involve 768-dimensional vectors (see Table \ref{tb:modelCharacteristics}).
In more detail, fastText and S-T5 are consistently the fastest and slowest models, respectively.

In figure \ref{fig:blk_time_real}, we can see the trade-off between effectiveness and efficiency. Each points holds the average time for each method across all datasets and the corresponding average recall. Since we want in each axis to achieve maximum score, we have normalized the y-axis of time by $min_{time} / time$. 

Thus, it is clear that paying more time yields higher recall for S-T5, but an alternative and more economic choice is S-MiniLM.

However, this overhead time is negligible in comparison to the vectorization time in Table \ref{tb:vectTime}. For this reason, the relative time efficiency remains the same as the one discussed in Section \ref{sec:vectorizonExp}.

\begin{figure}[!t]
\centering
\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.47\textwidth]{figures/blocking_real_vec_exact_agn_corr.pdf}
\vspace{-12pt}
% \caption{{\small Pearson correlation per pair of models wrt blocking~recall.}}
\caption{Pearson correlation of models wrt blocking recall.}
\label{fig:blk_heat_pear}
\vspace{-8pt}
\end{figure}

\input{tables/st5VsDeepBlocker}

% \textbf{Comparison to DeepBlocker.}

\begin{figure*}[!t]
\centering
\subfloat{\includegraphics[width=1.0\linewidth]{figures/blocking_synthetic_legend.pdf}}
\vspace{-7pt}
\setcounter{subfigure}{0}
% \newline
\subfloat[Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_recall_approx.pdf}\label{subfig:blk_synth_rec_app}}
\subfloat[Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_precision_approx.pdf}\label{subfig:blk_synth_pre_app}}
\subfloat[Blocking Time (sec-log)]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/blocking_synthetic_time_approx.pdf}\label{subfig:blk_synth_time_app}}
\subfloat[Vectorization  Time (sec-log)]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth]{figures/vectorization_synthetic_time.pdf}\label{subfig:vec_synth_time}}

\vspace{-12pt}
\caption{Scalability analysis over the synthetic datasets in Table \ref{tb:datasets}(b). The horizontal axis indicates the number of input entities.}
\label{fig:blk_synth}
\vspace{-15pt}
\end{figure*}

\subsection{Comparison to state-of-the-art}

We now compare the best performing language model, S-T5, with the state-of-the-art blocking approach that is based on deep learning and embeddings vectors: DeepBlocker's Auto-Encoder with FastText embeddings. The relative performance of the two methods over all datasets in Table \ref{tb:datasets}(a) appears in Table \ref{tb:st5vsdeepblocker} (including vectorization time for S-T5). Note that since DeepBlocker is a stochastic approach, we take the average of 10 runs.

\textbf{Effectiveness.}
S-T5 consistently outperforms DeepBlocker's recall to a significant extent. The only exceptions are $D_1$ and $D_4$, where both methods achieve practically perfect recall -- except for $k=1$, where S-T5 is marginally better, by 3\% and 1\%, respectively. The reason is that $D_1$ involves a very low number of duplicate pairs in relation to the size of each data source, while $D_4$ contains relatively clean entities with long textual descriptions that are easy to match.
In the remaining 8 datasets, the superiority of S-T5 is inversely proportional to the number of candidates per query entity, i.e., the lower $k$ is, the larger is the advantage of S-T5.

\textbf{Efficiency.}
DeepBlocker is consistently faster than S-T5 for $k$=1 and $k$=5 in all datasets but $D_{10}$.
The reason for the slow operation of S-T5 is its high vectorization cost, which accounts for $\sim$99\% of the overall blocking time. This explains why its run-time is practically stable per dataset across all values of $k$. This is expected, though, given that S-T5 leverages 768-dimensional embeddings vectors, compared to 300-dimensional FastText vectors of DeepBlocker. Yet, for $k$=10, DeepBlocker is faster than S-T5 only in $D_2$ and $D_3$ (by 14.4\% and 26\%, respectively). The situation is reversed in $D_1$ and $D_4$-$D_8$, where S-T5 is faster by 14.1\%, on average. The reason is that DeepBlocker does not scale well as the number of candidates per query entity increases, due to the high complexity of the deep neural network that lies at its core. Most importantly, DeepBlocker does scale well as the size of the input data increases: in $D_{10}$, S-T5 is faster by 1.5 times for $k \in \{1, 5\}$ and 3.7 times for $k$=10. This is further verified in Section~\ref{sec:scalability}.

\textbf{Summary.} 
Overall, we can conclude that S-T5 exhibits much higher blocking recall than DeepBlocker in all non-trivial cases at the cost of much higher overhead in case of small datasets and few candidates per query entity. In all other cases, S-T5 dominates DeepBlocker with respect to both effectiveness and time efficiency.




==> matching.tex <==
\section{Performance Comparison on Matching}

There are two methodologies for addressing matching \cite{DBLP:books/daglib/0030287,DBLP:journals/pvldb/GetoorM12}:
\begin{itemize}[leftmargin=*]
    \item \textit{Unsupervised Matching} is formalized as a clustering task, where the candidate pairs are organized into disjoint groups, such that each group corresponds to a different real-world object (i.e., all pairs within each group are matching).
    \item \textit{Supervised Matching} is formalized as a binary classification task, where the goal is to categorize the candidate pairs of blocking into two classes: \texttt{match} and \texttt{non-match}. Typically, a training set is used to learn a classification model, a validation set is used to choose its optimal configuration, and finally, a testing set is used to assess its performance on new, unknown instances. 
\end{itemize}

% The performance of language models on the former task is examined in Section \ref{sec:unsupMatching} and on the latter task in Section \ref{sec:supMatching}.

\begin{figure*}[!t]
\centering

% \subfloat{\includegraphics[width=0.6\linewidth]{figures/matching_real_legend.pdf}}
% \setcounter{subfigure}{0}
% \newline

\subfloat[D1 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D1_scores.pdf}}
\subfloat[D1 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D1_time.pdf}} 
%\hspace{5mm}%
\subfloat[D2 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D2_scores.pdf}}
\subfloat[D2 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D2_time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D3 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D3_scores.pdf}}
\subfloat[D3 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D3_time.pdf}} 
%\hspace{5mm}%
\subfloat[D4 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D4_scores.pdf}}
\subfloat[D4 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D4_time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D5 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D5_scores.pdf}}
\subfloat[D5 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D5_time.pdf}} 
%\hspace{5mm}%
\subfloat[D6 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D6_scores.pdf}}
\subfloat[D6 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D6_time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D7 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D7_scores.pdf}}
\subfloat[D7 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D7_time.pdf}} 
%\hspace{5mm}%
\subfloat[D8 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D8_scores.pdf}}
\subfloat[D8 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D8_time.pdf}}
\newline
\vspace{-12pt}
\subfloat[D9 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D9_scores.pdf}}
\subfloat[D9 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D9_time.pdf}} 
%\hspace{5mm}%
\subfloat[D10 / Scores]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D10_scores.pdf}}
\subfloat[D10 / Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=30mm]{figures/matching_real_D10_time.pdf}}
\newline
\vspace{-12pt}
\caption{{\color{myblue}Precision}, {\color{myorange}Recall}, {\color{mygreen}F1} and {\color{myred}Matching Time} for Unsupervised Matching per dataset in Table \ref{tb:datasets}(a).}
\vspace{-12pt}
\label{fig:match_unsup}
\end{figure*}

% \input{tables/supervisedMatching}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.27\textwidth]{figures/smPearson.png}
%     \vspace{-10pt}
%     \caption{Pearson correlation between the F1 of all models in Table \ref{tb:supMatching}.}
%     \label{fig:smPearson}
%     \vspace{-10pt}
% \end{figure}

% \begin{figure*}[!t]
% \centering
% \subfloat[Unsupervised]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_corr.pdf}\label{subfig:unsup_corr}}
% \subfloat[Supervised]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_corr.pdf}\label{subfig:sup_corr}}

% \caption{The correlation per pair of vectorizers for F1 for (a) unsupervised
% and (b) supervised for Matching.}
% \vspace{-12pt}
% \label{fig:match_corr}
% \end{figure*}

\begin{figure}[!t]
\centering
{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_corr.pdf}\label{subfig:sup_corr}}

\caption{Pearson correlation with respect to F1 per pair of language models for unsupervised matching.}
\vspace{-8pt}
\label{fig:match_corr}
\end{figure}

% \input{tables/smDatasets}

\subsection{Unsupervised Matching}
\label{sec:unsupMatching}

\begin{figure}[!t]
\centering
{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_heat.pdf}\label{subfig:match_unsup_heat}}
\vspace{-12pt}
\caption{The ranking position of each method per dataset in unsupervised settings for Matching. Lower is better.}
\vspace{-12pt}
\label{fig:matching_heat}
\end{figure}

% \begin{figure}[!t]
% \centering
% \subfloat[Supervised]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_heat.pdf}\label{subfig:match_sup_heat}}
% \newline
% \subfloat[Unsupervised]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_heat.pdf}\label{subfig:match_unsup_heat}}

% \caption{The ranking position of each method per dataset in (a) supervised
% and (b) unsupervised settings for Matching. Lower is better.}
% \label{fig:matching_heat}
% \end{figure}

% Results in Fig \ref{fig:match_unsup}.

We now examine the performance of all language models in the task of bipartite graph matching, i.e., in every dataset, each entity from the one data source is matched with at most one entity from the other data source.
% To this end, we performed the following experiments: for each dataset in Table \ref{}, we applied Blocking using the best language model from the experiment in Section , namely X. 
% We indexed the smallest dataset and queried with the entities of the largest one using $K$=10.
% For each of the resulting pair of candidates, we estimated the Euclidean similarity between the corresponding pre-trained vectors and applied Connected Components clustering using the optimal threshold, i.e., the thresholds that maximizes the F1 of each model in the range of [0,1] with a step of Z.
% Each component corresponds to a distinct entity.
% {\color{blue} Alex: Alternative description of above, more accurate:
% For each dataset, we want to match one entity from the left collection to exactly one of the right collection. Equivalently, we want to perform a greedy algorithm of Bipartite Matching. 
To this end, we apply Unique Mapping Clustering \cite{DBLP:conf/kdd/Lacoste-JulienPDKGG13}. We calculate all similarities between all pairs of entities and iterate over them in descending order of similarity score, 
{\color{blue} until all entities from the smallest data source are matched or, if a similarity threshold $\delta$ is defined, until there are no more pairs that exceed $\delta$.}
% until all entities from the smallest data source are matched or there are no more pairs that exceed the specified similarity threshold.
In this context, the current pair is marked as duplicates if none of its entities has already been matched with another entity.
% An entity is marked as matched when in an edge both entities are not matched. 
{\color{blue} After every examination of a pair, we could calculate precision and recall and find the corresponding F1 score. Note that there is an increasing trend in recall and a decreasing trend in precision, thus there is a point where the F1 score is maximized and this should be the best achievable performance for this model. It could be denoted by the current examined similarity, e.g. $\delta=0.87$ or the percentage of the entities matched in the smallest collection, e.g. 40\%. For example, a language model $LM_1$ can reach this peak after having matched 50\% of the entities in the smallest collection and the next similarity to be examined would be 0.83, while another language model $LM_2$ could have reached the corresponding peak while matching 80\% of the entities with scores = 0.97. Since it is not efficient to calculate these scores at every iteration, we do so in batches, i.e. every $\epsilon=0.05$ in pair similarities, starting from $\delta=0.95$.}

% This approach has an increasing trend for recall, but a decreasing trend in precision. 
% To maximize the effectiveness of each language model on every dataset, we consider all similarity thresholds in $[0, 1]$ with a step of 0.05 and select as optimal the one yielding the highest F1. 
% {\color{blue}Note that there is a point where F1 score is maximized and we can choose this point as the best performance for the language model, which will be different for each one. To avoid calculating precision and recall after every matching / examination of an edge, we do so in batches, after a step of $e=0.05$ in similarities, starting from $\delta=0.95$.  }

% Hence, we estimate the optimal performance in terms of F1 per language model by terminating as soon as 
% an optimized version is to pause the algorithm every Z steps and monitor how much F1 has changed. We either set a criterion to stop early or we run the algorithm exhaustively and afterwards select the point where the F1 was maximized.
% }

% The effectiveness of the outcomes are evaluated in terms of Recall (portion of matching pairs in the components), Precision (portion of matching pairs across all components) and F1 (the harmonic mean of Recall and Precision). The resulting performance along with clustering time, which assesses time efficiency, is presented in Figure \ref{fig:match_unsup}.. We observe that the language models can be distinguished into three groups. 

\textbf{Effectiveness.}
% The corresponding results are reported in 
Figure \ref{fig:match_unsup} reports the performance of all models with respect to
% to both effectiveness and time efficiency. The former includes 
recall, precision and f-measure (F1).
% , which is the harmonic mean of the two. 

The SentenceBERT models consistently dominate all others. The best one is \textsf{S-T5}, achieving the highest F1 in seven out of the 10 datasets. In the remaining datasets, it is ranked second or third, lying very close to the top performer. On average, its distance from the maximum F1 is just 0.7\%, being the lowest among all models. The worst case corresponds to $D_6$, where it lies 4.9\% lower than the best method. The second best model is \textsf{S-MiniLM}, having the highest F1 in three datasets and the second lowest average distance from the maximum F1 (6.5\%). The two next best models are \textsf{S-MPNet} and \textsf{S-DistilRoBERTa}, whose average distance from the top is 10.5\%.
% one by 
% , on average. 

% In both relative and absolute terms, their best performance  where their F1 is lower than the maximum one by $\sim$1\% and 0.7\%, respectively, whereas their worst performance is exhibited over $D_{10}$, where they underperform the top model by 30.6\% and 33.2\%, respectively. 

In absolute terms, their best performance 
% of these models 
corresponds to the bibliographic datasets, $D_4$ and $D_9$, where their F1 remains well over 0.9. 
% is almost perfect over $D_4$ and $D_9$, the two bibliographic datasets where 
The reason is that the long titles and list of authors facilitate the distinction between matching and non-matching entities. Also high ($\sim$0.8) is their F1 over $D_2$, which combines long textual descriptions with a 1-1 matching between the two data sources (i.e., every entity from the one source matches with one entity from the other). In all other datasets, their F1 ranges from 0.35 ($D_{10}$) to 0.77 ($D_7$), due to the high levels of noise they contain. 

The second best group of models corresponds to the static ones. Based on the average distance from the top, GloVe is the best one (31.9\%) followed by FastText (37.4\%) and Word2Vec (39.4\%). In absolute terms, their F1 remains rather low in all datasets except for the bibliographic ones: in $D_4$, it exceeds 0.9, lying very close to the SentenceBERT models, but in $D_9$, only FastText and Glove manage to surpass 0.7. The reason is that the entities from the Google Scholar are much more noisy and involve many more terminologies than $D_4$. In all other cases, their F1 falls (far) below 0.57. 

Finally, the BERT-based models form the group of the least effective models. The worst performance is consistently exhibited by XLNet and AlBERT, as their F1 does not exceed 0.37 in any dataset. On average, their F1 is almost an order of magnitude ($\sim$87\%) lower than the top one. In the other extreme lie DistilBERT and RoBERTa, with an average distance of $\sim$55\%. Finally, BERT fluctuates between these two extremes, with an average distance from the top equal to 62\%. These three models score an acceptable F1 ($\sim$0.9) in the clean and easy $D_4$, but remain (far) below 0.54 in all other cases. 

% The above observations are verified in Figure \ref{fig:matching_heat}, which summarizes the ranking position of each model per dataset.
Figure \ref{fig:matching_heat} summarizes the ranking position of each model per dataset.
The SentenceBERT models typically fluctuate between positions 1 and 4, the static ones between 5 and 7 and the BERT-based ones between 8 and 12. Moreover, the Pearson correlation of their F1 in Figure \ref{fig:match_corr} shows an almost perfect dependency between the Sentence-BERT models and a very high one inside the group of static and BERT-based ones. The latter
% , especially XLNet and AlBERT,
are weakly correlated with the SentenceBERT models. The static models have moderate correlation $(0.7-0.9)$ with the other two groups.

% Overall, we can conclulde that the BERT-based models require fine-tuning in order to be able to distinguish between the matching and the non-matching entities. The static models outperform them because they are independent of fine-tuning, but underperform the SentenceBERT ones, which are capable of enriching their embeddings with contextual positional evidence.
{\color{blue} Overall, we can corroborate the finding in \cite{reimers2019sentence} that the BERT-based models perform even worse than static models when they are not fine-tuned. Moreover, the static models underperform the SentenceBERT ones, which are capable of enriching their embeddings with contextual positional evidence.
}

% The first one includes the high performing models, which are the following (in decreasing order of average F1, as shown in Figure X(b): S-T5, S-MINILM, S-MPNet, S-DistilRoBERTa. Their difference in terms of average F1 is significant ({\color{red}CHECK!!}), but rather low, ranging between 0.5X and 0.6Y across all datasets. They all excel in Recall, which on average exceeds 0.8 for all of them. They suffer, though, from low Precision, which is rather unstable, but fluctuates around 0.5, on average. For both measures, these models consistently outperform all others.

\textbf{Efficiency.} Time efficiency is assessed in terms of matching time ($t_m$), i.e., the time that is required for applying the Unique Mapping Clustering algorithm to all pairwise similarities using the optimal pruning threshold.
% {\color{red}[Dimitris: Some comments on efficiency, and also a summary here?]}
Its matching time is typically much lower than half a second, except the largest dataset, $D_{10}$, where it raises to almost two seconds. This high efficiency in the context of a large number of candidate pairs should be attributed to its rather high similarity threshold, which fluctuates between 0.55 and 0.70, with a median (mean) of 0.625 (0.615), thus pruning the vast majority of pairs.
Its lower effectiveness is combined with a much higher time efficiency. Even though its pruning threshold is lower by 0.05 or 0.10 than that of \textsf{S-T5} -- except for $D_1$, where it is higher by 0.05 --- its matching time is significantly lower in most cases. In fact, it is faster than \textsf{S-T5} by 3, 10 and 5 times over $D_1$, $D_3$ and $D_{10}$, respectively.
Their pruning thresholds are typically lower than \textsf{S-T5}, fluctuating between 0.50 and 0.65, thus yielding higher run-times. Yet, the matching time of \textsf{S-DistilRoBERTa} is consistently lower than a second, due to the distillation it conveys, while \textsf{S-MPNet} takes $\sim$3 minutes to process $D_{10}$.

\textbf{Comparison to the state-of-the-art.} In this experiment we wanted to test an end-to-end framework of the best model so far, i.e. S-T5. To do so, we have used the matching algorithm described above, but instead of utilizing all pairs of entities, each query entity is allowed only $k$ candidates, produced by Blocking. We have compared our framework with ZeroER \cite{wu2020zeroer}. As it can be seen in Table \ref{tb:zeroer}, ZeroER was not able to terminate in most datasets and in the rest cases, the blocking time was much larger than the total execution time of S-T5. In terms of effectiveness, again results are mostly in favor of S-T5, with the exception of D5, where S-T5 has a very low performance.

% , which 

% \begin{figure*}[!t]
% \centering
% \subfloat[F1]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_euclidean_f1.pdf}\label{subfig:match_unsup_eucl_f1}}
% \subfloat[Precision]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_euclidean_precision.pdf}\label{subfig:match_unsup_eucl_pre}}
% \newline
% \subfloat[Recall]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_euclidean_recall.pdf}\label{subfig:match_unsup_eucl_rec}}
% \subfloat[Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_euclidean_time.pdf}\label{subfig:match_unsup_eucl_time}}

% \caption{Matching Statistics when unsupervised for euclidean similarity.}
% \label{fig:match_unsup}
% \end{figure*}

% \begin{figure*}[!t]
% \centering
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D1_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D1_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D2_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D2_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D3_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D3_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D4_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D4_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D5_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D5_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D6_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D6_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D7_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D7_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D8_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D8_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D9_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D9_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D10_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.40\textwidth, height=2cm]{figures/matching_real_D10_time.pdf}}
% \newline
% \caption{Precision, Recall, F1 and Matching Time for Unsupervised Matching from real data per case.}
% \label{fig:match_unsup}
% \end{figure*}

% \begin{figure*}[!t]
% \centering

% \subfloat{\includegraphics[width=0.6\linewidth]{figures/matching_real_legend.pdf}}
% \setcounter{subfigure}{0}
% % \newline

% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D1_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D1_time.pdf}} 
% %\hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D2_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D2_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D3_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D3_time.pdf}} 
% %\hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D4_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D4_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D5_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D5_time.pdf}} 
% %\hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D6_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D6_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D7_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D7_time.pdf}} 
% %\hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D8_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D8_time.pdf}}
% \newline
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D9_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D9_time.pdf}} 
% %\hspace{5mm}%
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D10_scores.pdf}}
% \subfloat{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.25\textwidth, height=2cm]{figures/matching_real_D10_time.pdf}}
% \newline
% \caption{Precision, Recall, F1 and Matching Time for Unsupervised Matching from real data per case.}
% \label{fig:match_unsup}
% \end{figure*}








% \begin{table*}[]
% \begin{tabular}{|l|r|r|l|l|r|r|}
% \hline
%  & \multicolumn{1}{c|}{\textbf{simple\_accuracy}} & \multicolumn{1}{l|}{\textbf{f1}} & \textbf{model\_type} & \textbf{data\_dir} & \multicolumn{1}{l|}{\textbf{training\_time}} & \multicolumn{1}{l|}{\textbf{testing\_time}} \\ \hline
% \textbf{0} & 0.981481 & 0.961538 & roberta & dirty\_amazon\_itunes & 66.449704 & 0.417442 \\ \hline
% \textbf{1} & 0.972846 & 0.865979 & roberta & abt\_buy & 1773.642234 & 11.178319 \\ \hline
% \textbf{2} & 0.966797 & 0.830846 & roberta & dirty\_walmart\_amazon & 1111.16982 & 6.832608 \\ \hline
% \textbf{3} & 0.993528 & 0.981818 & roberta & dirty\_dblp\_acm & 1548.867166 & 9.608327 \\ \hline
% \textbf{4} & 0.983452 & 0.956201 & roberta & dirty\_dblp\_scholar & 2665.860271 & 15.763607 \\ \hline
% \textbf{5} & 0.777778 & 0.142857 & bert & dirty\_amazon\_itunes & 66.374553 & 0.421454 \\ \hline
% \textbf{6} & 0.89295 & 0.009662 & bert & abt\_buy & 1761.490139 & 11.20175 \\ \hline
% \textbf{7} & 0.90625 & 0 & bert & dirty\_walmart\_amazon & 1094.100369 & 6.827322 \\ \hline
% \textbf{8} & 0.837783 & 0.176591 & bert & dirty\_dblp\_acm & 1526.566565 & 9.610102 \\ \hline
% \textbf{9} & 0.941996 & 0.818331 & bert & dirty\_dblp\_scholar & 2616.337042 & 15.797002 \\ \hline
% \textbf{10} & 0.907407 & 0.791667 & distilbert & dirty\_amazon\_itunes & 34.013834 & 0.209837 \\ \hline
% \textbf{11} & 0.962402 & 0.817259 & distilbert & abt\_buy & 892.516487 & 5.501003 \\ \hline
% \textbf{12} & 0.948242 & 0.719577 & distilbert & dirty\_walmart\_amazon & 559.746822 & 3.398238 \\ \hline
% \textbf{13} & 0.996764 & 0.990971 & distilbert & dirty\_dblp\_acm & 779.428393 & 4.765573 \\ \hline
% \textbf{14} & 0.980143 & 0.946729 & distilbert & dirty\_dblp\_scholar & 1342.018722 & 7.909392 \\ \hline
% \textbf{15} & 0.916667 & 0.830189 & sdistilroberta & dirty\_amazon\_itunes & 31.3895 & 0.189659 \\ \hline
% \textbf{16} & 0.971279 & 0.861461 & sdistilroberta & abt\_buy & 810.718882 & 4.99689 \\ \hline
% \textbf{17} & 0.958984 & 0.79 & sdistilroberta & dirty\_walmart\_amazon & 518.768934 & 3.071899 \\ \hline
% \textbf{18} & 0.992718 & 0.97973 & sdistilroberta & dirty\_dblp\_acm & 718.553671 & 4.311861 \\ \hline
% \textbf{19} & 0.983452 & 0.955793 & sdistilroberta & dirty\_dblp\_scholar & 1253.022755 & 7.088994 \\ \hline
% \textbf{20} & 0.935185 & 0.857143 & sminilm & dirty\_amazon\_itunes & 25.452475 & 0.14696 \\ \hline
% \textbf{21} & 0.971279 & 0.857143 & sminilm & abt\_buy & 721.548304 & 4.198407 \\ \hline
% \textbf{22} & 0.944336 & 0.738532 & sminilm & dirty\_walmart\_amazon & 417.236195 & 2.322793 \\ \hline
% \textbf{23} & 0.997168 & 0.992126 & sminilm & dirty\_dblp\_acm & 580.766968 & 3.309804 \\ \hline
% \textbf{24} & 0.979794 & 0.945845 & sminilm & dirty\_dblp\_scholar & 997.42478 & 5.291353 \\ \hline
% \textbf{25} & 0.953704 & 0.893617 & albert & dirty\_amazon\_itunes & 62.953257 & 0.452219 \\ \hline
% \textbf{26} & 0.965535 & 0.833333 & albert & abt\_buy & 1691.875594 & 12.001003 \\ \hline
% \textbf{27} & 0.971191 & 0.843501 & albert & dirty\_walmart\_amazon & 1026.218671 & 7.330419 \\ \hline
% \textbf{28} & 0.995955 & 0.988713 & albert & dirty\_dblp\_acm & 1447.356514 & 10.324953 \\ \hline
% \textbf{29} & 0.980665 & 0.947765 & albert & dirty\_dblp\_scholar & 2420.552547 & 16.97863 \\ \hline
% \textbf{30} & 0.981481 & 0.961538 & smpnet & dirty\_amazon\_itunes & 61.358782 & 0.392012 \\ \hline
% \textbf{31} & 0.972324 & 0.861619 & smpnet & abt\_buy & 1636.612695 & 10.505692 \\ \hline
% \textbf{32} & 0.966309 & 0.823529 & smpnet & dirty\_walmart\_amazon & 1006.388176 & 6.29032 \\ \hline
% \textbf{33} & 0.995955 & 0.988764 & smpnet & dirty\_dblp\_acm & 1409.782391 & 8.899997 \\ \hline
% \textbf{34} & 0.982059 & 0.952381 & smpnet & dirty\_dblp\_scholar & 2412.954589 & 14.436873 \\ \hline
% \textbf{35} & 0.944444 & 0.892857 & xlnet & dirty\_amazon\_itunes & 92.347872 & 0.69287 \\ \hline
% \textbf{36} & 0.971279 & 0.863524 & xlnet & abt\_buy & 2916.313126 & 24.193804 \\ \hline
% \textbf{37} & 0.950684 & 0.760095 & xlnet & dirty\_walmart\_amazon & 1425.830889 & 10.155074 \\ \hline
% \textbf{38} & 0.995146 & 0.986486 & xlnet & dirty\_dblp\_acm & 2123.29039 & 15.866718 \\ \hline
% \textbf{39} & 0.982407 & 0.952914 & xlnet & dirty\_dblp\_scholar & 3203.332697 & 20.865489 \\ \hline
% \end{tabular}
% \caption{Statistics for supervised matching}
% \end{table*}


% \begin{tabular}{llrrrr}
% \toprule
%     &       &    time &  recall &  precision &    f1 \\
% case & col &         &         &            &       \\
% \midrule
% D1 & aggregate value &   17.39 &    1.00 &       0.03 &  0.05 \\
%     & name &   14.34 &    1.00 &       0.03 &  0.05 \\
%     & phone\_number &   17.22 &    0.95 &       0.02 &  0.05 \\
% D2 & aggregate value &   17.31 &    0.66 &       0.07 &  0.12 \\
%     & description &   17.46 &    0.17 &       0.02 &  0.03 \\
%     & name &   16.85 &    0.83 &       0.08 &  0.15 \\
% D3 & aggregate value &   35.57 &    0.62 &       0.05 &  0.09 \\
%     & description &   35.46 &    0.40 &       0.03 &  0.06 \\
%     & title &   25.88 &    0.90 &       0.07 &  0.14 \\
% D4 & aggregate value &   27.83 &    1.00 &       0.08 &  0.16 \\
%     & authors &   27.30 &    0.98 &       0.08 &  0.15 \\
%     & title &   31.75 &    1.00 &       0.08 &  0.16 \\
% D5 & aggregate value &   62.48 &    0.80 &       0.02 &  0.03 \\
%     & name &   55.59 &    0.52 &       0.01 &  0.02 \\
%     & title &   59.68 &    0.47 &       0.01 &  0.02 \\
% D6 & aggregate value &   68.34 &    0.95 &       0.02 &  0.03 \\
%     & name &   65.28 &    0.29 &       0.01 &  0.01 \\
%     & title &   64.77 &    0.69 &       0.01 &  0.02 \\
% D7 & aggregate value &   49.42 &    0.85 &       0.03 &  0.06 \\
%     & name &   52.42 &    0.48 &       0.02 &  0.04 \\
%     & title &   46.24 &    0.51 &       0.02 &  0.04 \\
% D8 & aggregate value &   46.05 &    0.86 &       0.03 &  0.06 \\
%     & modelno &   34.18 &    0.64 &       0.02 &  0.04 \\
%     & title &   41.69 &    0.84 &       0.03 &  0.05 \\
% D9 & aggregate value &  270.38 &    0.91 &       0.08 &  0.15 \\
%     & authors &  241.63 &    0.67 &       0.06 &  0.11 \\
%     & title &  241.64 &    0.95 &       0.09 &  0.16 \\
% D10 & aggregate value &  371.40 &    0.40 &       0.03 &  0.06 \\
%     & starring &  283.16 &    0.07 &       0.01 &  0.01 \\
%     & title &  280.69 &    0.56 &       0.05 &  0.09 \\
% \bottomrule
% \end{tabular}








% \begin{table*}

% \begin{tabular}{lrrrrrrrrrr}
% \toprule
% {} & \multicolumn{5}{l}{ZeroER} & \multicolumn{5}{l}{S5} \\
% {} & Blocking (sec) & Matching (sec) & Precision & Recall &    F1 & Vectorization Time & Matching Time & Recall & Precision &    F1 \\
% Dataset &                &                &           &        &       &                    &               &        &           &       \\
% \midrule
% D1      &           2.12 &           0.38 &      0.00 &   0.00 &  0.00 &              12.44 &          0.48 &   0.99 &      0.26 &  0.41 \\
% D2      &        1727.55 &          70.70 &      0.86 &   0.32 &  0.46 &              20.21 &          0.15 &   0.83 &      0.83 &  0.83 \\
% D3      &            NaN &            NaN &       NaN &    NaN &   NaN &              47.92 &          1.40 &   0.64 &      0.52 &  0.58 \\
% D4      &        9595.28 &         113.19 &      0.97 &   0.97 &  0.97 &              25.97 &         11.79 &   0.98 &      0.95 &  0.97 \\
% D5      &        1291.44 &           9.77 &      0.91 &   0.95 &  0.93 &              45.73 &         17.03 &   0.75 &      0.16 &  0.26 \\
% D6      &            NaN &            NaN &       NaN &    NaN &   NaN &              61.91 &         66.75 &   0.88 &      0.16 &  0.27 \\
% D7      &        1598.54 &         338.19 &      0.86 &   0.90 &  0.88 &              41.03 &         28.27 &   0.90 &      0.35 &  0.50 \\
% D8      &            NaN &            NaN &       NaN &    NaN &   NaN &              92.97 &          9.10 &   0.69 &      0.23 &  0.35 \\
% D9      &            NaN &            NaN &       NaN &    NaN &   NaN &             197.02 &          8.94 &   0.95 &      0.87 &  0.91 \\
% D10     &            NaN &            NaN &       NaN &    NaN &   NaN &              98.66 &        369.65 &   0.49 &      0.48 &  0.48 \\
% \bottomrule
% \end{tabular}

% \caption{Statistics for ZeroER, Schema-Agnostic}
% \end{table*}


\begin{table}
\setlength{\tabcolsep}{1.8pt}
\small
\begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|}

\hline
{} & \multicolumn{5}{|c|}{ZeroER} & \multicolumn{5}{|c|}{S-T5} \\
\hline
Dataset & BLK & MTCH  & Prec. & Rec. &    F1 & VECT & MTCH & Rec. & Prec. &    F1 \\
\hline
\hline
D1      &           2.12 &           0.38 &      0.00 &   0.00 &  0.00 &              12.44 &          0.00 &   0.99 &      0.32 &  0.48 \\
D2      &        1727.55 &          70.70 &      0.86 &   0.32 &  0.46 &              20.21 &          0.00 &   0.82 &      0.85 &  0.83 \\
D3      &            - &            - &       - &    - &   - &              47.92 &          0.00 &   0.64 &      0.52 &  0.57 \\
D4      &        9595.28 &         113.19 &      0.97 &   0.97 &  0.97 &              25.97 &          0.01 &   0.98 &      0.97 &  0.97 \\
D5      &        1291.44 &           9.77 &      0.91 &   0.95 &  0.93 &              45.73 &          0.01 &   0.74 &      0.20 &  0.31 \\
D6      &            - &            - &       - &    - &   - &              61.91 &          0.02 &   0.87 &      0.21 &  0.34 \\
D7      &        1598.54 &         338.19 &      0.86 &   0.90 &  0.88 &              41.03 &          0.01 &   0.90 &      0.47 &  0.62 \\
D8      &            - &            - &       - &    - &   - &              92.97 &          0.01 &   0.69 &      0.24 &  0.35 \\
D9      &            - &            - &       - &    - &   - &             197.02 &          0.01 &   0.95 &      0.88 &  0.91 \\
D10     &            - &            - &       - &    - &   - &              98.66 &          0.09 &   0.49 &      0.55 &  0.52 \\
\hline
\end{tabular}



% \caption{Comparison between ZeroER and S-T5 for Schema-Agnostic in terms of time (sec) and efficiency}
\caption{ZeroER vs S-T5 on Unsupervised Matching.}
\label{tb:zeroer}
\vspace{-15pt}
\end{table}


\input{tables/supervisedMatching}
\input{tables/supervisedMatchingEfficiency}

\subsection{Supervised Matching}
\label{sec:supMatching}

To examine the performance of all models in the task of supervised matching, we combine them with \textit{EMTransformer} \cite{DBLP:conf/edbt/BrunnerS20}. We selected this approach among the open-source deep learning-based matching algorithms, because it achieves state-of-the-art performance, while relying exclusively on the embedding models. This is in contrast to DITTO \cite{DBLP:journals/pvldb/0001LSDT20}, which leverages external information, such as POS tagging. This is also in contrast to DeepMatcher \cite{Mudgal2018sigmod}, which is crafted for the static models, unlike EMTransformer, which supports dynamic ones, too. In fact, the static language models are excluded from this analysis, because their representations cannot be adjusted after training. As a result, they are incompatible with EMTransformer. \textsf{S-T5} is also excluded, because it follows the Encoder-Decoder architecture, which is different than the other models which only have the Encoder component. 
% the dynamic language models, unlike the various classifiers produced by 

% fine-tunes each model using a training set to maximize their performance. 
The original implementation of EMTransformer disregards the validation set and evaluates each model directly on the testing set. However, this results in overfitting, as noted in \cite{DBLP:journals/corr/abs-2004-00584}. We modified the code so that it follows the standard approach in the literature: for each trained model, the validation set is used to check whether it maximizes F1 and this model is then applied to the testing set \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}. 
For this analysis, we used the five datasets shown in Table~\ref{tb:smDatasets}.
% {\color{red}We used the same five datasets as in 
% \cite{DBLP:conf/edbt/BrunnerS20}, which are widely used in the literature} \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}. Their technical characteristics are reported in Table \ref{tb:smDatasets}; 60\% of all pairs form the training set, while the rest are equally split between the validation and test set. {\color{red}Note that most of them stem from the datasets in Table \ref{tb:rlDatasets}}: $DSM_1$ is part of $D_2$, $DSM_3$ of $D_4$, $DSM_4$ of $D_9$ and $DSM_5$ of $D_8$. The only exception is $DSM_2$, which is not included in Table \ref{tb:rlDatasets}, due to the lack of its complete groundtruth. Note also that $DSM_2$-$DSM_5$ are \textit{dirty datasets} in the sense that they include artificial noise in the form of missing and misplaced attribute values \cite{DBLP:journals/pvldb/0001LSDT20}. The goal of these settings is to increase their difficulty.


\textbf{Effectiveness.}
Table \ref{tb:supMatching} summarizes the results of our experiments with respect to effectiveness (F1 score) over the datasets in Table \ref{tb:smDatasets} (the best performance per dataset is highlighted in bold). As baseline methods we have included the performance of DITTO and DeepMatcher, as reported in \cite{DBLP:journals/pvldb/0001LSDT20}.
We observe that RoBERTa is the most robust model in terms of effectiveness. 
% As shown in Figure \ref{fig:matching_heat}(a), 
It achieves the highest F1 in most datasets, ranking first on average. In fact, the mean distance from the top F1 across all datasets amounts to just 0.5\%. It is followed in close distance by the second best model, S-MPNet, which is top performer in one dataset ($DSM_3$) and its average distance from the top F1 is 0.7\%.  
The rest of the models are sorted in the following order according to their average distance from the top performance: BERT, AlBERT, XLNet, S-DistilRoBERTa, S-MiniLM. 

Even the least effective model, though, is just 5\% worse than the best one, on average. The reason for this is the strong correlation between all considered models: high effectiveness for one model on a specific dataset implies similarly high effectiveness for the rest of the models. This pattern should be partially attributed to the $DSM_3$ and $DSM_4$ datasets, where the difference between the maximum and the minimum F1 is less than 1.3\%. These datasets convey relatively clean values, even though in both cases artificial noise has been inserted in the form of misplaced values. This means that the duplicate entities share multiple common tokens in the schema-agnostic settings we are considering. As a result, even classic machine learning classifiers that use string similarity measures as features achieve very high F1 ($>$0.9) in these datasets (see Magellan in \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}). The rest of the datasets are more challenging, due to the terminologies they involve (e.g., product names). As a result, the difference between the maximum and minimum F1 of these models ranges from 4.9\% ($DSM_1$) to 
% 12.4\% ($DSM_5$) and 
17\% ($DSM_2$).

These experiments indicate that the BERT-based models match and even outwit the SentenceBERT ones, unlike for the blocking and the unsupervised matching tasks, due to the fine-tuning of their last layer.

% Note that there is a strong dependency in the performance of the various models: high effectiveness for one model on a specific dataset implies similarly high effectiveness for the rest of the models. This is verified in {\color{red}Figure \ref{fig:smPearson}}, which reports the Pearson correlation $\rho$ with respect to F1 between all pairs of models. With the exception of BERT, for all other models $\rho \geq 0.73$, reaching the maximum value for two pairs: RoBERTa \& S-MPNet and DistilBERT \& S-DistilRoBERTa. 

% {\color{red}Add a few phrases that justify the relative performance of these models.}

\textbf{Efficiency.}
% {\color{red}[Dimitris: Some comments on efficiency, and also a summary here?]}
%while the corresponding 
We report the time efficiency of the language models with respect to training time ($t_t$) and testing time ($t_r$) 
% is reported 
in Table \ref{tb:supMatchingTime}. We observe that S-MPNet constitutes the best choice for applications that emphasize time efficiency at the cost of slightly lower effectiveness: its training and prediction time are consistently lower than that of RoBERTa by 8.7\% and 7.2\%, respectively, on average.
Compared to XLNet, which is consistently the slowest model in all respects among all datasets, RoBERTa excels in both effectiveness and run-time, as it is faster by $\geq38\%$, on average. ALBERT achieves slightly lower training times (by 6.7\%) than RoBERTa at the cost of higher prediction times (by 7.6\%). The rest of the models reduce both run-times to a half, on average, at the cost of significantly lower F1 ($\ll$10\%).

\textbf{Comparison to the state-of-the-art.} Comparing the language models to DeepMatcher+, which leverages FastText embeddings, we observe that they outperform it in practically all cases. This is particularly true in $DSM_1$ and $DSM_5$, where the worst language model (DistilBERT) exceeds DeepMatcher+ by $\sim$20\%. DITTO, on the other hand, is directly comparable to the best performing language model in each dataset. In $DSM_2$, $DSM_3$ and $DSM_4$, DITTO's F1 is lower by just $\leq$0.5\%. In $DSM_1$ and $DSM_5$, though, DITTO outperforms all language models
% to a significant extent, 
by 3\% and 1.5\%, respectively. This should be attributed to the external knowledge and the data augmentation. The effect of these features is more clear when comparing DITTO to the language model that lies at its core, i.e., RoBERTa. On average, across all datasets, the latter underperforms DITTO by 1.3\%. 
% This is counterbalanced, though, by the much lower training time, due to the lower number of epochs required by EMTransformer.

% Results in Fig \ref{fig:match_sup}.

% \begin{figure*}[!t]
% \centering
% \subfloat[ABT - BUY]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_ABT_BUY.pdf}\label{subfig:match_sup_abt_buy}}
% \subfloat[Dirty Amazon - Itunes]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_AMAZON_ITUNES.pdf}\label{subfig:match_sup_amazon_itunes}}
% \newline
% \subfloat[Dirty DBLP - ACM]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_DBLP_ACM.pdf}\label{subfig:match_sup_dblp_acm}}
% \subfloat[Dirty DBLP - Scholar]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_DBLP_SCHOLAR.pdf}\label{subfig:match_sup_dblp_scholar}}
% \newline
% \subfloat[Dirty Walmart - Amazon]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_WALMART_AMAZON.pdf}\label{subfig:match_sup_walmart_amazon}}

% \caption{Matching Statistics when supervised}
% \label{fig:match_sup}
% \end{figure*}





==> matching_2.tex <==
\section{Performance Comparison on Matching}

There are two methodologies for addressing matching \cite{DBLP:books/daglib/0030287,DBLP:journals/pvldb/GetoorM12}:
\begin{itemize}[leftmargin=*]
    \item \textit{Unsupervised Matching} is formalized as a clustering task, where the candidate pairs are organized into disjoint groups, such that each group corresponds to a different real-world object (i.e., all pairs within each group are matching).
    \item \textit{Supervised Matching} is formalized as a binary classification task, where the goal is to categorize the candidate pairs of blocking into two classes: \texttt{match} and \texttt{non-match}. Typically, a training set is used to learn a classification model, a validation set is used to choose its optimal configuration, and finally, a testing set is used to assess its performance on new, unknown instances. 
\end{itemize}

\begin{figure*}[!t]
\centering
\subfloat[Static]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/unsup_matching_static.pdf}} 
\subfloat[BERT]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/unsup_matching_BERT.pdf}}
\subfloat[SBERT]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.33\textwidth, height=40mm]{figures/unsup_matching_SBERT.pdf}} 
\caption{F1 in Unsupervised Matching per group of methods from real data.}
\vspace{-12pt}
\label{fig:match_unsup_rec_real}
\end{figure*}

\begin{figure}[!t]
\centering
\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.50\textwidth]{figures/unsup_matching_pareto.pdf} 
\caption{Pareto Front for F1 and Matching Time (sec) per method from real data.}
\vspace{-12pt}
\label{fig:match_unsup_time_real}
\end{figure}



\begin{figure}[!t]
\centering
{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_corr.pdf}\label{subfig:sup_corr}}

\caption{Pearson correlation with respect to F1 per pair of language models for unsupervised matching.}
\vspace{-8pt}
\label{fig:match_corr}
\end{figure}

% \input{tables/smDatasets}

\subsection{Unsupervised Matching}
\label{sec:unsupMatching}

\begin{figure}[!t]
\centering
{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_unsupervised_heat.pdf}\label{subfig:match_unsup_heat}}
\vspace{-12pt}
\caption{The ranking position of each method per dataset in unsupervised settings for Matching. Lower is better.}
\vspace{-12pt}
\label{fig:matching_heat}
\end{figure}


We now examine the performance of all language models in the task of bipartite graph matching, i.e., in every dataset, each entity from the one data source is matched with at most one entity from the other data source.
To this end, we apply Unique Mapping Clustering \cite{DBLP:conf/kdd/Lacoste-JulienPDKGG13}. We calculate all similarities between all pairs of entities and iterate over them in descending order of similarity score, 
{\color{blue} until all entities from the smallest data source are matched or, if a similarity threshold $\delta$ is defined, until there are no more pairs that exceed $\delta$.}
In this context, the current pair is marked as duplicates if none of its entities has already been matched with another entity.
{\color{blue} After every examination of a pair, we could calculate precision and recall and find the corresponding F1 score. Note that there is an increasing trend in recall and a decreasing trend in precision, thus there is a point where the F1 score is maximized and this should be the best achievable performance for this model. It could be denoted by the current examined similarity, e.g. $\delta=0.87$ or the percentage of the entities matched in the smallest collection, e.g. 40\%. For example, a language model $LM_1$ can reach this peak after having matched 50\% of the entities in the smallest collection and the next similarity to be examined would be 0.83, while another language model $LM_2$ could have reached the corresponding peak while matching 80\% of the entities with scores = 0.97. Since it is not efficient to calculate these scores at every iteration, we do so in batches, i.e. every $\epsilon=0.05$ in pair similarities, starting from $\delta=0.95$.}


\textbf{Effectiveness.}
Figure \ref{fig:match_unsup_rec_real} reports the performance of all models with respect to f-measure (F1).

$\bullet$ In static models, based on the average distance from the top, GloVe is the best one (31.9\%) followed by FastText (37.4\%) and Word2Vec (39.4\%). In absolute terms, their F1 remains rather low in all datasets except for the bibliographic ones: in $D_4$, it exceeds 0.9, lying very close to the SentenceBERT models, but in $D_9$, only FastText and Glove manage to surpass 0.7. The reason is that the entities from the Google Scholar are much more noisy and involve many more terminologies than $D_4$. In all other cases, their F1 falls (far) below 0.57. 

$\bullet$ In the BERT-based models, the worst performance is consistently exhibited by XLNet and AlBERT, as their F1 does not exceed 0.37 in any dataset. On average, their F1 is almost an order of magnitude ($\sim$87\%) lower than the top one. {\color{red} The reasons are probably the same as in Blocking: Both were trained for a different task and cannot perform well in the task of Matching, without further fine-tuning.}. In the other extreme lie DistilBERT and RoBERTa, with an average distance of $\sim$55\%. Finally, BERT fluctuates between these two extremes, with an average distance from the top equal to 62\%. These three models score an acceptable F1 ($\sim$0.9) in the clean and easy $D_4$, but remain (far) below 0.54 in all other cases. 

$\bullet$ In the SentenceBERT models, the best one is \textsf{S-T5}, achieving the highest F1 in seven out of the 10 datasets. In the remaining datasets, it is ranked second or third, lying very close to the top performer. On average, its distance from the maximum F1 is just 0.7\%, being the lowest among all models. The worst case corresponds to $D_6$, where it lies 4.9\% lower than the best method. The second best model is \textsf{S-MiniLM}, having the highest F1 in three datasets and the second lowest average distance from the maximum F1 (6.5\%). The two next best models are \textsf{S-MPNet} and \textsf{S-DistilRoBERTa}, whose average distance from the top is 10.5\%.


In absolute terms, their best performance 
corresponds to the bibliographic datasets, $D_4$ and $D_9$, where their F1 remains well over 0.9. 
The reason is that the long titles and list of authors facilitate the distinction between matching and non-matching entities. Also high ($\sim$0.8) is their F1 over $D_2$, which combines long textual descriptions with a 1-1 matching between the two data sources (i.e., every entity from the one source matches with one entity from the other). In all other datasets, their F1 ranges from 0.35 ($D_{10}$) to 0.77 ($D_7$), due to the high levels of noise they contain. 


$\bullet$ Finally, between groups, we can claim that again S-T5 was better than the best of the other two groups, since with the exception of $D_4$, all other models do not surpass 0.5 in F1. On the contrary with the task of Blocking, though, in Matching we can perform fine-tuning to detect if BERT models can, indeed, perform better than static ones. This will be the object of section \ref{sec:supMatching}.


\textbf{Summary.} 
Figure \ref{fig:matching_heat} summarizes the ranking position of each model per dataset.
The SentenceBERT models typically fluctuate between positions 1 and 4, the static ones between 5 and 7 and the BERT-based ones between 8 and 12. Moreover, the Pearson correlation of their F1 in Figure \ref{fig:match_corr} shows an almost perfect dependency between the Sentence-BERT models and a very high one inside the group of static and BERT-based ones. The latter
are weakly correlated with the SentenceBERT models. The static models have moderate correlation $(0.7-0.9)$ with the other two groups.

\textbf{Efficiency.} Time efficiency is assessed in terms of matching time ($t_m$), i.e., the time that is required for applying the Unique Mapping Clustering algorithm to all pairwise similarities using the optimal pruning threshold.
Its matching time is typically much lower than half a second, except the largest dataset, $D_{10}$, where it raises to almost two seconds. This high efficiency in the context of a large number of candidate pairs should be attributed to its rather high similarity threshold, which fluctuates between 0.55 and 0.70, with a median (mean) of 0.625 (0.615), thus pruning the vast majority of pairs.
Again, we can see the trade-off in Figure \ref{fig:unsup_matching_pareto}, where S-T5 offers the best F1 with the second worse average time across all datasets and S-MiniLM being the most economic in regard of time.

{color{red}Alex: Not sure these two paragraphs should be kept without the corresponding bigger figure:}
Its lower effectiveness is combined with a much higher time efficiency. Even though its pruning threshold is lower by 0.05 or 0.10 than that of \textsf{S-T5} -- except for $D_1$, where it is higher by 0.05 --- its matching time is significantly lower in most cases. In fact, it is faster than \textsf{S-T5} by 3, 10 and 5 times over $D_1$, $D_3$ and $D_{10}$, respectively.
Their pruning thresholds are typically lower than \textsf{S-T5}, fluctuating between 0.50 and 0.65, thus yielding higher run-times. Yet, the matching time of \textsf{S-DistilRoBERTa} is consistently lower than a second, due to the distillation it conveys, while \textsf{S-MPNet} takes $\sim$3 minutes to process $D_{10}$.


\textbf{Comparison to the state-of-the-art.} In this experiment we wanted to test an end-to-end framework of the best model so far, i.e. S-T5. To do so, we have used the matching algorithm described above, but instead of utilizing all pairs of entities, each query entity is allowed only $k$ candidates, produced by Blocking. We have compared our framework with ZeroER \cite{wu2020zeroer}. As it can be seen in Table \ref{tb:zeroer}, ZeroER was not able to terminate in most datasets and in the rest cases, the blocking time was much larger than the total execution time of S-T5. In terms of effectiveness, again results are mostly in favor of S-T5, with the exception of D5, where S-T5 has a very low performance.


\begin{table}
\setlength{\tabcolsep}{1.8pt}
\small
\begin{tabular}{|c|r|r|r|r|r|r|r|r|r|r|}

\hline
{} & \multicolumn{5}{|c|}{ZeroER} & \multicolumn{5}{|c|}{S-T5} \\
\hline
Dataset & BLK & MTCH  & Prec. & Rec. &    F1 & VECT & MTCH & Rec. & Prec. &    F1 \\
\hline
\hline
D1      &           2.12 &           0.38 &      0.00 &   0.00 &  0.00 &              12.44 &          0.00 &   0.99 &      0.32 &  0.48 \\
D2      &        1727.55 &          70.70 &      0.86 &   0.32 &  0.46 &              20.21 &          0.00 &   0.82 &      0.85 &  0.83 \\
D3      &            - &            - &       - &    - &   - &              47.92 &          0.00 &   0.64 &      0.52 &  0.57 \\
D4      &        9595.28 &         113.19 &      0.97 &   0.97 &  0.97 &              25.97 &          0.01 &   0.98 &      0.97 &  0.97 \\
D5      &        1291.44 &           9.77 &      0.91 &   0.95 &  0.93 &              45.73 &          0.01 &   0.74 &      0.20 &  0.31 \\
D6      &            - &            - &       - &    - &   - &              61.91 &          0.02 &   0.87 &      0.21 &  0.34 \\
D7      &        1598.54 &         338.19 &      0.86 &   0.90 &  0.88 &              41.03 &          0.01 &   0.90 &      0.47 &  0.62 \\
D8      &            - &            - &       - &    - &   - &              92.97 &          0.01 &   0.69 &      0.24 &  0.35 \\
D9      &            - &            - &       - &    - &   - &             197.02 &          0.01 &   0.95 &      0.88 &  0.91 \\
D10     &            - &            - &       - &    - &   - &              98.66 &          0.09 &   0.49 &      0.55 &  0.52 \\
\hline
\end{tabular}



\caption{ZeroER vs S-T5 on Unsupervised Matching.}
\label{tb:zeroer}
\vspace{-15pt}
\end{table}


\input{tables/supervisedMatching}
\input{tables/supervisedMatchingEfficiency}

\subsection{Supervised Matching}
\label{sec:supMatching}

To examine the performance of all models in the task of supervised matching, we combine them with \textit{EMTransformer} \cite{DBLP:conf/edbt/BrunnerS20}. We selected this approach among the open-source deep learning-based matching algorithms, because it achieves state-of-the-art performance, while relying exclusively on the embedding models. This is in contrast to DITTO \cite{DBLP:journals/pvldb/0001LSDT20}, which leverages external information, such as POS tagging. This is also in contrast to DeepMatcher \cite{Mudgal2018sigmod}, which is crafted for the static models, unlike EMTransformer, which supports dynamic ones, too. In fact, the static language models are excluded from this analysis, because their representations cannot be adjusted after training. As a result, they are incompatible with EMTransformer. \textsf{S-T5} is also excluded, because it follows the Encoder-Decoder architecture, which is different than the other models which only have the Encoder component. 
% the dynamic language models, unlike the various classifiers produced by 

% fine-tunes each model using a training set to maximize their performance. 
The original implementation of EMTransformer disregards the validation set and evaluates each model directly on the testing set. However, this results in overfitting, as noted in \cite{DBLP:journals/corr/abs-2004-00584}. We modified the code so that it follows the standard approach in the literature: for each trained model, the validation set is used to check whether it maximizes F1 and this model is then applied to the testing set \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}. 
For this analysis, we used the five datasets shown in Table~\ref{tb:smDatasets}.
% {\color{red}We used the same five datasets as in 
% \cite{DBLP:conf/edbt/BrunnerS20}, which are widely used in the literature} \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}. Their technical characteristics are reported in Table \ref{tb:smDatasets}; 60\% of all pairs form the training set, while the rest are equally split between the validation and test set. {\color{red}Note that most of them stem from the datasets in Table \ref{tb:rlDatasets}}: $DSM_1$ is part of $D_2$, $DSM_3$ of $D_4$, $DSM_4$ of $D_9$ and $DSM_5$ of $D_8$. The only exception is $DSM_2$, which is not included in Table \ref{tb:rlDatasets}, due to the lack of its complete groundtruth. Note also that $DSM_2$-$DSM_5$ are \textit{dirty datasets} in the sense that they include artificial noise in the form of missing and misplaced attribute values \cite{DBLP:journals/pvldb/0001LSDT20}. The goal of these settings is to increase their difficulty.


\textbf{Effectiveness.}
Table \ref{tb:supMatching} summarizes the results of our experiments with respect to effectiveness (F1 score) over the datasets in Table \ref{tb:smDatasets} (the best performance per dataset is highlighted in bold). As baseline methods we have included the performance of DITTO and DeepMatcher, as reported in \cite{DBLP:journals/pvldb/0001LSDT20}.
We observe that RoBERTa is the most robust model in terms of effectiveness. 
% As shown in Figure \ref{fig:matching_heat}(a), 
It achieves the highest F1 in most datasets, ranking first on average. In fact, the mean distance from the top F1 across all datasets amounts to just 0.5\%. It is followed in close distance by the second best model, S-MPNet, which is top performer in one dataset ($DSM_3$) and its average distance from the top F1 is 0.7\%.  
The rest of the models are sorted in the following order according to their average distance from the top performance: BERT, AlBERT, XLNet, S-DistilRoBERTa, S-MiniLM. 

Even the least effective model, though, is just 5\% worse than the best one, on average. The reason for this is the strong correlation between all considered models: high effectiveness for one model on a specific dataset implies similarly high effectiveness for the rest of the models. This pattern should be partially attributed to the $DSM_3$ and $DSM_4$ datasets, where the difference between the maximum and the minimum F1 is less than 1.3\%. These datasets convey relatively clean values, even though in both cases artificial noise has been inserted in the form of misplaced values. This means that the duplicate entities share multiple common tokens in the schema-agnostic settings we are considering. As a result, even classic machine learning classifiers that use string similarity measures as features achieve very high F1 ($>$0.9) in these datasets (see Magellan in \cite{DBLP:journals/pvldb/0001LSDT20,Mudgal2018sigmod}). The rest of the datasets are more challenging, due to the terminologies they involve (e.g., product names). As a result, the difference between the maximum and minimum F1 of these models ranges from 4.9\% ($DSM_1$) to 
% 12.4\% ($DSM_5$) and 
17\% ($DSM_2$).

These experiments indicate that the BERT-based models match and even outwit the SentenceBERT ones, unlike for the blocking and the unsupervised matching tasks, due to the fine-tuning of their last layer.

% Note that there is a strong dependency in the performance of the various models: high effectiveness for one model on a specific dataset implies similarly high effectiveness for the rest of the models. This is verified in {\color{red}Figure \ref{fig:smPearson}}, which reports the Pearson correlation $\rho$ with respect to F1 between all pairs of models. With the exception of BERT, for all other models $\rho \geq 0.73$, reaching the maximum value for two pairs: RoBERTa \& S-MPNet and DistilBERT \& S-DistilRoBERTa. 

% {\color{red}Add a few phrases that justify the relative performance of these models.}

\textbf{Efficiency.}
% {\color{red}[Dimitris: Some comments on efficiency, and also a summary here?]}
%while the corresponding 
We report the time efficiency of the language models with respect to training time ($t_t$) and testing time ($t_r$) 
% is reported 
in Table \ref{tb:supMatchingTime}. We observe that S-MPNet constitutes the best choice for applications that emphasize time efficiency at the cost of slightly lower effectiveness: its training and prediction time are consistently lower than that of RoBERTa by 8.7\% and 7.2\%, respectively, on average.
Compared to XLNet, which is consistently the slowest model in all respects among all datasets, RoBERTa excels in both effectiveness and run-time, as it is faster by $\geq38\%$, on average. ALBERT achieves slightly lower training times (by 6.7\%) than RoBERTa at the cost of higher prediction times (by 7.6\%). The rest of the models reduce both run-times to a half, on average, at the cost of significantly lower F1 ($\ll$10\%).

\textbf{Comparison to the state-of-the-art.} Comparing the language models to DeepMatcher+, which leverages FastText embeddings, we observe that they outperform it in practically all cases. This is particularly true in $DSM_1$ and $DSM_5$, where the worst language model (DistilBERT) exceeds DeepMatcher+ by $\sim$20\%. DITTO, on the other hand, is directly comparable to the best performing language model in each dataset. In $DSM_2$, $DSM_3$ and $DSM_4$, DITTO's F1 is lower by just $\leq$0.5\%. In $DSM_1$ and $DSM_5$, though, DITTO outperforms all language models
% to a significant extent, 
by 3\% and 1.5\%, respectively. This should be attributed to the external knowledge and the data augmentation. The effect of these features is more clear when comparing DITTO to the language model that lies at its core, i.e., RoBERTa. On average, across all datasets, the latter underperforms DITTO by 1.3\%. 
% This is counterbalanced, though, by the much lower training time, due to the lower number of epochs required by EMTransformer.

% Results in Fig \ref{fig:match_sup}.

% \begin{figure*}[!t]
% \centering
% \subfloat[ABT - BUY]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_ABT_BUY.pdf}\label{subfig:match_sup_abt_buy}}
% \subfloat[Dirty Amazon - Itunes]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_AMAZON_ITUNES.pdf}\label{subfig:match_sup_amazon_itunes}}
% \newline
% \subfloat[Dirty DBLP - ACM]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_DBLP_ACM.pdf}\label{subfig:match_sup_dblp_acm}}
% \subfloat[Dirty DBLP - Scholar]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_DBLP_SCHOLAR.pdf}\label{subfig:match_sup_dblp_scholar}}
% \newline
% \subfloat[Dirty Walmart - Amazon]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/matching_supervised_DIRTY_WALMART_AMAZON.pdf}\label{subfig:match_sup_walmart_amazon}}

% \caption{Matching Statistics when supervised}
% \label{fig:match_sup}
% \end{figure*}





==> scalabilityAnalysis.tex <==
\subsection{Scalability Analysis}
\label{sec:scalability}

% \input{tables/syntheticDatasets}

Blocking must scale to large data volumes in order to restrict the input of matching to manageable levels, even in cases 
% where the input comprises 
with millions of entities.
% profiles. 
Therefore, we need to assess how well the selected language models scale as the size of the input data increases. 

% To this end, we employ the seven datasets in Table \ref{tb:dedupDatasets}, which are widely used in the literature for the same purpose \cite{DBLP:journals/pvldb/0001SGP16,DBLP:journals/is/KenigG13,DBLP:journals/tkde/Christen12}. They were artificially generated by Febrl \cite{DBLP:conf/kdd/Christen08a}, in the following way: clean records were initially created by extracting real names (given and surname) and addresses (street number,
% name, postcode, suburb, and state names) from frequency tables of real census data. 
% Next, duplicate records were randomly generated according to realistic error rates and types (e.g., by inserting, deleting or replacing characters or words).
% In the end result, 40\% of all records are matching with at least another one. There are at most 9 duplicates per record and up to 3 and 10 modifications per attribute value and record,~resp.

To this end, we conduct an analysis using the seven datasets shown in Table \ref{tb:datasets}(b).
These correspond to \textit{Dirty ER}, a.k.a., Deduplication, where a single data source containing duplicates is given as input \cite{DBLP:series/synthesis/2021Papadakis,DBLP:series/synthesis/2015Christophides}.
{\color{blue} Here, due to the large dataset size, we use approximate instead of exact nearest neighbor search. To do so, based on \cite{li2019approximate} we chose to utilize an HNSW \cite{DBLP:journals/pami/MalkovY20} index, which is a state-of-the-art algorithm for this task. More specifically, an HNSW index is a graph-based index, serving as an approximation to a Delaunay graph, but with long-range links as well, to support the small-world navigation property. To avoid the issue of high-degree nodes in the original NSW and possible connectivity issues, the Hierarchical NSW introduces a multi-layer separation of links based on the degree and an advanced heuristic to better select the neighbors of each node. To be noted, a graph-based a-NNS index offers very good querying times with the tradeoff of a large overhead in building the index. In our experiments we used the implementation in FAISS \footnote{https://faiss.ai/cpp_api/struct/structfaiss_1_1IndexHNSW.html}. Specifically, 
after vectorizing the input dataset as in Section \ref{sec:vectorizonExp}, we index all entities using FAISS(HNSW); then, we query the resulting index with every entity $e$ in order to retrieve the $k$=10 approximate nearest neighbors in terms of Euclidean distance -- excluding $e$. The results appear in Figure \ref{fig:blk_synth}.}



% This means that every entity is a possible match with any other entity.
% Here, due to the large dataset size, we use approximate instead of exact nearest neighbor search, applying FAISS \cite{DBLP:journals/tbd/JohnsonDJ21} in combination with HNSW \cite{DBLP:journals/pami/MalkovY20}, which is a state-of-the-art algorithm for this task. Specifically, 
% % we perform blocking as follows:
% % actually consider the following settings for each model:
% after vectorizing the input dataset as in Section \ref{sec:vectorizonExp}, we index all entities using FAISS(HNSW); then, we query the resulting index with every entity $e$ in order to retrieve the $k$=10 approximate nearest neighbors in terms of Euclidean distance -- excluding $e$.
% % , exhibiting one of the highest throughput in answering queries~\cite{DBLP:journals/is/AumullerBF20}.
% % Nwe consider . 
% % The resulting performance with respect to effectiveness and time efficiency appears in Figure \ref{fig:blk_synth}.
% The results appear in Figure \ref{fig:blk_synth}.

\textbf{Effectiveness.}
% Starting with recall i
In Figure \ref{fig:blk_synth}(a), we observe that recall consistently decreases for all models as we move from $D_{10K}$ to $D_{2M}$. This is expected, given that the number of candidates increases quadratically with the size of the input data. The best performance clearly corresponds to S-T5: its recall over $D_{2M}$ is quite satisfactory both in absolute terms (0.800) and in relation to the initial one over $D_{10K}$ (0.962), as it drops by just 17\%. The second best approach in most datasets is FastText, whose recall is reduced by 54\%, from 0.901 to 0.415. On the other extreme lie AlBERT and XLNet: their recall is lower than 0.18 across all datasets (even for $D_{10K}$) and is reduced by 2/3 over $D_{2M}$. The rest of the models fluctuate between these two extremes and can be arranged into three groups according to their performance. The best group comprises S-DistilRoberta and S-MiniLM, which start from $\sim$0.750 over the smallest dataset and end up $\sim$40\% lower at 0.450. The worst group
% , which exhibits significantly lower performance than the previous one, 
includes Word2Vec, DistilBERT, BERT and RoBERTa, whose recall drops by 56\%-66\%, falling far below 0.2 over $D_{2M}$. GloVe and S-MPNet are located in the middle of the first two extremes: their recall is reduced by less than 50\% and exceeds 0.32 over $D_{2M}$.

We observe almost the same patterns with respect to precision in Figure \ref{fig:blk_synth}(b). This is due to the linear relation between the two measures, as explained earlier.
% in Dirty ER: precision shares the same numerator as recall (i.e., the number of detected duplicates), while the denominator is almost identical across all models, due to the same number of candidates that are fetched for each entity ($k=10$). 
Only minor variations occur in the context of Dirty ER, due to the different number of redundant candidate pairs, which are counted once (a candidate pair $<$$e_i$, $e_j$$>$ is redundant if $e_j$ is included in the nearest neighbors of $e_i$ and vice versa). Hence, there is a gradual decrease in precision for all models as the input size increases. This is larger than the decrease in recall by 2-3\% in most cases, because the denominator of recall (i.e., the number of existing duplicates) increases at a slower pace than the denominator of precision (i.e., number of distinct candidate pairs).
% The difference in the erosion of precision and recall raises to 7\% and 6\% for the two most effective models, S-T5 and FastText, respectively; the former (latter) starts from 0.112 (0.091) over $D_{10K}$ and decreases gradually, dropping by 24\% (60\%) to 0.085 (0.037) over $D_{2M}$. This indicates that the two models produce less redundant pairs as the input size increases.

\textbf{Efficiency.}
% Regarding the 
% overhead
% execution
% time i
In Figure \ref{fig:blk_synth}(c), we observe that the execution time scales superlinearly, but subquadratically in all cases: as the number of input increases by 200 times from $D_{10K}$ to $D_{2M}$, the run-times increase by up to 1,435 times. With the exception of the two most efficient models, Word2Vec (742 times) and S-T5 (873 times), all other models fluctuate between 1,053 (SMPNet) and 1,435 (XLNet) times.
% There are two reasons for this superlinearity:
% \begin{enumerate}[leftmargin=*]
%     \item The very low run-time over the smallest dataset, as all models process $D_{10K}$ in far less than 1 second. The slowest model is actually S-T5, which requires 850 milliseconds. 
%     % Note that for S-T5, the highest starting point allows it to achieve the second lowest increase in run-time, as explained above.{\color{red}[Dimitris: this is not clear to me.]}
%     \item FAISS(HNSW) trades high indexing time for significantly lower querying time. During indexing, it actually performs complex graph-based operations that involve long paths. The larger the input size, the longer these paths get, increasing the cost of their traversal and processing. Hence, the indexing time dominates the total time, with querying accounting for a small portion.
% \end{enumerate}
This is mainly attributed to the fact that FAISS(HNSW) trades high indexing time for significantly lower querying time. During indexing, it requires complex graph-based operations that involve long paths. The larger the input size, the longer these paths get, increasing the cost of their traversal and processing. Hence, the indexing time dominates the total time.
% , with querying accounting for a small portion.

Finally, Figure \ref{fig:blk_synth}(d) reports the evolution of vectorization time, which increases sublinearly with the size of the input data. The increase fluctuates between 127 (DistilBERT) and 165 (XLNet) times for all BERT-based models, thus remaining far below  the raise in the input size (i.e., 200 from $D_{10K}$ to $D_{2M}$). A similar behavior is exhibited by S-T5, but the rest of the SentenceBERT models achieve even better scalability, as their increase is reduced to 59 (S-MiniLM), 94 (S-MPNet) and 62 (XLNet). All these models are outperformed by the two most efficient static ones, Word2Vec and GloVe, which raise their run-times by just 2.5 and 4 times, respectively. The former actually remains practically stable up to $D_{300K}$, because its vectorization time is dominated by its high initialization time across the five smallest datasets. On the other extreme lies FastText, which is the only model that scales linearly with the size of the input data (i.e., its vectorization time increases by 205 from $D_{10K}$ to $D_{2M}$).
% {\color{red}This should be attributed to its extreme efficiency over the smallest dataset, where it achieves the lowest run-time by far among all models.}

In absolute terms, GloVe is consistently the fastest model in all datasets, but $D_{10K}$, with Word2Vec ranking second from $D_{200K}$ on. They vectorize $D_{2M}$ within 0.8 and 1.3 minutes, respectively. FastText is the second fastest model for the three smallest datasets, but converges to the fastest dynamic model, S-MiniLM, for the larger ones. They both need $\sim$11 minutes to process $D_{2M}$. On the other extreme lies S-T5, which consistently exhibits the slowest vectorization, with XLNet being the second worst model across all datasets. For $D_{2M}$, they take 90.3 and 50.6 minutes, respectively. The rest of the models
% fluctuate between these two extremes, but 
can be grouped in three pairs: the slowest one, which is faster only than XLNet, includes BERT and RoBERTa, which vectorize $D_{2M}$ within 34.6 and 31.9 minutes, respectively. The middle pair involves DistiBERT and S-MPNet, with the former being faster than the latter by 16\%, on average ($\sim$25 minutes over $D_{2M}$). The fastest pair comprises S-MiniLM and S-DistilRoBERTa, with the former outperforming the latter by 15\%, on average. These observations verify the conclusions drawn from Section \ref{sec:vectorizonExp} about the relative vectorization time of the considered models.

% \input{tables/scalabilityDeepblocker}

\textbf{Comparison to the state-of-the-art.} We applied DeepBlocker's Auto-Encoder with FastText embeddings to the datasets in Table \ref{tb:datasets}(b). However, it runs out of memory already for the third largest dataset, due to its quadratic space complexity (i.e., it tries to create % it they requires ∼300GB of RAM to create 
a 100K×100K float array for $D_{100K}$). 
For $D_{10K}$ it takes 39.4 sec and scores 0.749 in recall and 0.130 in precision, whereas in $D_{50K}$ it takes 463.2 sec and scores 0.676 and 0.116 accordingly. As a result,
%Table \ref{tb:DeepBlockerScal} shows
DeepBlocker is $\sim$5\% slower than S-T5 in $D_{50K}$, while its recall is lower by $\sim$22\%. The superiority of S-T5 is wider in $D_{100K}$, where DeepBlocker is almost $\sim$3 times slower while yielding a recall lower by $\sim$28\%. FastText also outperforms DeepBlocker in all respects: it is an order of magnitude faster, while its recall is higher by at least 15\%. S-MiniLM and S-DistilRoBERTa exhibit a recall similar to DeepBlocker in both datasets, while being faster by $\sim$3 times and an order of magnitude over $D_{10K}$ and $D_{50K}$, respectively. All other models are much faster, but less effective than DeepBlocker.


\textbf{Summary.}
% {\color{red}[Dimitris: Can we add a short summary here?]}
S-T5 is the clear winner among all models, due to its robust recall, which is maintained at acceptable levels for $k$=10 despite raising the input size by 200 times. Its precision also remains at very high levels for blocking. On average, 1 out of 10 candidate pairs involves duplicate entities. On the downside, its overall run-time is the highest among all models. Yet, it processes the largest dataset within $\sim$1.5 hours, while it scales sub-linearly, increasing by just 164 times from $D_{10K}$ to $D_{2M}$, as it is dominated by the vectorization time. S-T5 also scales much better than DeepBlocker.

==> vectorization.tex <==
\section{Performance Comparison on Vectorization}
\label{sec:vectorizonExp}

% {\color{red}TODO: Alexandre, add a different boxplot diagram for schema-agnostic and schema-based settings.}

Vectorization is the task of converting every textual entity in a given dataset into its embedding vector. In the schema-agnostic setting we consider,
% every language model receives as input the sentence describing each entity and automatically returns the corresponding vector.
% FastText, for instance, 
%utilizing the feature of FastText to handle and 
% internally splits the sentence into smaller n-grams and aggregates their embeddings into a representative vector.
% The only exceptions are 
% Regarding the use of the models, 
% @Alexandros: Any comments about the use of the Huffing Face and Gensim implementations of the embeddings?}
% Word2Vec and GloVe, which exclusively provide token embeddings. Thus, we tokenize the original sentence into words and then average the word embeddings. 
we represent each entity by a ``sentence'' that is formed by concatenating all its textual attributes. For Word2Vec and GloVe, which only support word embeddings, we tokenize this sentence into words and average their vectors to obtain a single one. FastText internally splits the sentence into smaller n-grams and aggregates their embeddings into a single vector. The rest of the models generate an embedding for the entire sentence.

\textbf{Initialization.} 
The initialization time of each model is shown in the first line of Table~\ref{tb:vectTime}. It refers to the time taken to load the necessary data structures in main memory (e.g., a dictionary for the static models and a learned neural network for the dynamic ones), and is independent of the dataset used.
% We observe a high fluctuation among the considered models, {\color{blue} with the static models being the most inefficient ones by far. This should be attributed to the hash table that they load into main memory in order to map each token to an embedding vector.}
The static models are inefficient due to the hash table they need to load into main memory to map tokens to embedding vectors.
Regarding the dynamic models, we observe that the BERT-based ones are much faster than the SentenceBERT ones, as their average run-time is 4.7$\pm$0.8 and 8.9$\pm$0.6 seconds, respectively. This is due to the larger and more complex neural models that are used by the latter.


%with the Word2Vec and FastText being the most inefficient ones by far. This should be attributed to the hash table that they load into main memory in order to map each token to an embedding vector. 
%Given that FastText considers n-grams, its dictionary is much larger than that of Word2Vec, which exclusively considers tokens, and thus, FastText's initialization is more time consuming. The fastest static model is GloVe, {\color{blue}due to the implementation we used, which is provided by SBERT}.
%{\color{blue}The static models have on average a fast execution time, 2.9$\pm$5.4, with the exception of FastText in the last datasets, which is expected, since they have more and larger sentences and FastText splits each sentence and word into n-grams.} 

\textbf{Transformation.} 
The rest of Table~\ref{tb:vectTime} shows the total time required by each model to convert the entities of each dataset. Word2Vec and Glove are the fastest models by far, exhibiting the lowest processing run-times in practically all cases. Word2Vec is an order of magnitude faster than the third most efficient model per dataset, which interchangeably corresponds to FastText and S-MiniLM. Except for $D_1$, GloVe outperforms these two models by at least 6 times. In absolute terms, both Word2Vec and GloVe process the eight smallest datasets, $D_1$-$D_8$, in much less than 1 second, while requiring less than 2.5 seconds for the two larger ones.

Among the BERT-based models, DistilBERT is significantly faster than BERT, as expected, with its processing time being lower by 33\%, on average. Note, though, that it is slower than FastText by $>$50\%, on average, except for $D_3$. The next most efficient models of this category are ALBERT and RoBERTa, which outperform BERT by 11\% and 13\%, on average, respectively.
% On the other extreme lies
XLNet
% , which 
is the most time consuming BERT-based model, being slower than BERT by $\sim$30\%, on average across all datasets but $D_3$. This can be explained by the fact that $D_3$ has larger sentences, as shown in Table \ref{tb:datasets}.

\input{tables/vectTime}

% {\color{red}Can we explain why D3 is the exception in these cases?}

Regarding the SentenceBERT models, the lowest time is achieved by S-MiniLM, which, as mentioned above, is the third fastest model together with FastText.
% -- their difference is much lower than 1 second in seven of the datasets.
The second best model in this category is S-DistilRoBERTa, which is slower by 30\%, on average. Both models are faster than BERT
% to a large extent -- 
by 63\% and 53\%, respectively, on average.
% -- {\color{red}because they are inherently crafted for maximizing time efficiency.}
In contrast, the quite complex learned model of S-T5 yields the highest processing time among all models in all datasets but the smallest one. S-MPNet lies between these two extremes.
% , exhibiting a processing time similar to BERT in three datasets, but on average, it is faster than it by 14\%.

\textbf{Summary.} 
The static models excel in processing time, but suffer from very high initialization time. More notably, FastText is the slowest model in all datasets, but $D_9$, where S-T5 exhibits a much higher processing time. This means that FastText's high initialization cost does not pay off in datasets with few thousand entities like those in Table \ref{tb:datasets}(a). On average, FastText requires 2 minutes per dataset. All other models vectorize all datasets in less than 1 minute, with very few exceptions: BERT over $D_9$, XLNet over $D_9$-$D_{10}$ and S-T5 over $D_8$-$D_{10}$.


% \textbf{Summary.} 
% {The static models excel in processing time, but suffer from very high initialization time. \color{blue}In fact, GloVe consistently exhibits the fastest vectorization (i.e., overall) time across all models; the only exception is $D_1$, where DistilBERT is half a second faster, due to its lower initialization time. In contrast, FastText is the slowest model in all datasets, but $D_9$, where S-T5 exhibits a much higher processing time. This means that FastText's high initialization cost does not pay off in datasets with few thousand entities like those in Table \ref{tb:datasets}(a). On average, FastText requires 2 minutes per dataset. All other models vectorize all datasets in less than 1 minute, with very few exceptions: BERT over $D_9$, XLNet over $D_9$-$D_{10}$ and S-T5 over $D_8$-$D_{10}$.}


% Our goal is to assess the time efficiency of vectorization per language model, using the
% % of the language models, we examined the time taken to convert all entity profiles in the 
% datasets in Table \ref{tb:rlDatasets}.
% % into embeddings vectors. 
% More precisely, we measure the \textit{vectorization time}, which
% % and 
% is defined it as the sum of the \textit{initialization} and the \textit{processing time}, denoted by $t_i$ and $t_p$ respectively. The former corresponds to the average time taken to load the necessary data structures in main memory (e.g., a dictionary for the static models and a learned neural network for the dynamic ones). The latter is the total time required per dataset for the conversion of its entities.
% % in the 
% % schema-based and the 
% % schema-agnostic settings we are considering.

% This means that $t_i$ is common across all datasets. 
% % The initialization time per model 
% It appears in the first line of Table \ref{tb:vectTime}. We observe a high fluctuation among the considered models, with Word2Vec and FastText being the most inefficient ones by far. This should be attributed to the hash table that they load into main memory in order to map each token to an embedding vector. Given that FastText considers n-grams, its dictionary is much larger than that of Word2Vec, which exclusively considers tokens, and thus, FastText's initialization is more time consuming. The fastest static model is GloVe, {\color{red}because it...ALEXANDRE PLEASE FILL IN.} Regarding the dynamic models, we observe that the BERT-based ones are much faster than the SentenceBERT ones, as their average run-time is 4.7$\pm$0.8 and 8.9$\pm$0.6 seconds, respectively. This is apparently caused by the larger and more complex neural models that are used by the SentenceBERT models.

% % The vectorization time per language model appears in Figures \ref{fig:vec}(a) and (b) for the schema-agnostic and the schema-based settings. 
% % Starting with the former settings, 
% Regarding $t_p$, we observe that Word2Vec and Glove constitute the fastest models by far, exhibiting the lowest average processing run-times in practically all cases. Word2Vec is actually a whole order of magnitude faster than the third most efficient model per dataset, which interchangeably corresponds to FastText and S-MINILM. Except for $D_1$, GloVe outperforms these two models by at least 6 times. In absolute terms, both Word2Vec and GloVe process the eight smallest datasets, $D_1$-$D_8$, in much less than 1 second, while requiring less than 2.5 seconds for the two~larger~ones.

% Among the BERT-based models, DistilBERT is significantly faster than BERT, as expected, with its processing time being lower by 33\%, on average.
% % , and so does its deviation across all datasets. 
% Note, though, that it is slower than FastText by $>$50\%, on average, except for $D_3$. The next most efficient models of this category are ALBERT and RoBERTa, which outperform BERT by 11\% and 13\%, on average, respectively. On the other extreme lies XLNet, which is the most time consuming BERT-based model: it is slower than BERT by $\sim$30\%, on average across all datasets but $D_3$.
% % ; it is also the less robust model, as it exhibits the largest differences across the 10 datasets.

% {\color{red}Can we explain why D3 is the exception in these cases?}

% Regarding the SentenceBERT models, the lowest average $t_p$ is achieved by S-MiniLM, which, as mentioned above, is the third fastest model together with FastText -- their difference is much lower than 1 second in seven of the datasets. The second best model in this category is S-DistilRoBERTa, which is slower by 30\%, on average. Both models are faster than BERT to a large extent -- by 63\% and 53\%, respectively, on average -- {\color{red}because they are inherently crafted for maximizing time efficiency.} In contrast, the quite complex learned model of S-T5 yields the highest processing time among all models in all datasets but the smallest one. S-MPNet lies between these two extremes, exhibiting a processing time similar to BERT in three datasets, but on average, it is faster than it~by~14\%.

% % Similar patterns arise from the schema-based settings. The performance of three models (Glove, word2vec, XLNet) is practically the same in terms of average run-time, while all other models reduce it to a significant extent, i.e., by more than 10\% -- except for ALBERT, which improves by just 6\%. Their relative performance, though, remains almost identical: Glove is again the fastest among all models, followed by fastText and DistilBERT, which retain the second and third place, respectively. S-MINILM and S-DistilRoBERTa are still much faster than BERT, and so does ALBERT, though to a smaller extent. Most importantly, S-MPNet converges to BERT, due to its very high improvement (by 33\%), which is lower only to S-T5's improvements (70\%), which is now the second slowest model, after word2vec.

% On the whole, the static models excel in processing time, but they suffer from very high initialization time, except for GloVe. In fact, GloVe consistently exhibits the fastest vectorization (i.e., overall) time across all models; the only exception is $D_1$, where DistilBERT is half a second faster, due to its lower initialization time. In contrast, FastText is the slowest model in all datasets, but $D_9$, where S-T5 exhibits a much higher processing time. This means that FastText's high initialization cost does not pay off in datasets with few thousand entities like those in Table \ref{tb:rlDatasets}. On average, FastText requires 2 minutes per dataset. All other models vectorize all datasets in less than 1 minute, with very few exceptions: BERT over $D_9$, XLNet over $D_9$-$D_{10}$ and S-T5 over $D_8$-$D_{10}$.

% the schema-settings affect the performance of most models to a significant extent, as the vectorized text is much shorter in the case of specific attribute values. Yet, the relative performance is affected to a much lower extent: Glove and fastText are quite fast, while word2vec excels in scalability. These static models are followed by models leveraging techniques for increasing time efficiency, like distillation.

% \begin{figure*}[!t]
% \centering
% \subfloat[Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_real_time.pdf}\label{subfig:vec_real_time}}
% \subfloat[Memory]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_real_memory.pdf}\label{subfig:vec_real_memory}}
% \caption{Vectorization Statistics from real data.}
% \label{fig:vec_real}
% \end{figure*}

% \begin{figure}[!t]
% \centering
% % \subfloat[Real]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_real_time.pdf}\label{subfig:vec_real}}
% % \subfloat[Synthetic]{
% \includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.47\textwidth]{figures/vectorization_synthetic_time.pdf}
% % }
% \vspace{-8pt}
% \caption{Scalability analysis of vectorization time per model.}
% % \label{fig:vec}
% \label{fig:vec_synth}
% \end{figure}

% \subsubsection{Scalability analysis}

% Results in Fig \ref{fig:vec_synth}.

% \begin{figure*}[!t]
% \centering
% \subfloat[Time]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_synthetic_time.pdf}\label{subfig:vec_synth_time}}
% \subfloat[Memory]{\includegraphics[trim=0.12cm 0.12cm 0.12cm 0.12cm, clip, width=0.4\textwidth]{figures/vectorization_synthetic_memory.pdf}\label{subfig:vec_synth_memory}}
% \caption{Vectorization Statistics from synthetic data.}
% \label{fig:vec_synth}
% \end{figure*}
